Blind Map Level Systematics Cleaning: A Quadratic Estimator Approach

We present the first detailed case study using quadratic estimators (QE) to diagnose and remove systematics present in observed Cosmic Microwave Background (CMB) maps. In this work we focus on the temperature to polarization leakage. We use an iterative QE analysis to remove systematics, in analogy to de-lensing, recovering the primordial B-mode signal and the systematic maps. We introduce a new Gaussian filtering scheme crucial to stable convergence of the iterative cleaning procedure and validate with comparisons to semi-analytical forecasts. We study the limitations of this method by examining its performance both on idealized simulations and on more realistic, non-ideal simulations, where we assume varying de-lensing efficiencies. Finally, we quantify the systematic cleaning efficiency by presenting a likelihood analysis on the tensor to scalar ratio, $r$, and demonstrate that the blind cleaning results in an un-biased measurement of $r$, reducing the systematic induced B-mode power by nearly two orders of magnitude.

==> sections/acknowledgements.tex <==
\begin{acknowledgments}
JW and NM are supported by Science and Technology Facilities Council (STFC) studentships. DBT acknowledges support from  STFC grant ST/P000649/1. AR acknowledges support from...
\end{acknowledgments}


==> sections/mapsim.tex <==
\section{Map level systematic simulations \label{sec:mapsim}}

==> sections/old_files/qe.tex <==
\section{Quadratic estimators}
\label{sec:qe}
As discussed in section \ref{sec:recap} in this paper we consider a temperature to polarisation leakage induced by a gain mismatch between detectors. The nature of the temperature to polarization leakage, and indeed all of the distortions considered in \eqref{eqn:Distortion Fields}, as perturbative terms makes it possible to reconstruct these fields using quadratic estimators. This is in analogy to lensing reconstruction, where quadratic estimators are applied to the CMB fields to reconstruct the lensing potential \cite{2003PhRvD..68h3002H}

\subsection{Off diagonal correlations}
Normally all correlations between two harmonic space CMB fields, for example the auto-correlation of the $E$-mode polarization $\ensave{E_{lm}E^{*}_{l'm'}}$ or the cross-correlation between the temperature and $E$-mode polarization fields $\ensave{T_{lm}E^{*}_{l'm'}}$, are on diagonal.\NM{MLB Comment - Is this true also on the cut sky? } That is, for these correlations only terms where $l=l'$ are non-zero. This is true for all Gaussian random variables.
However, distortions of the real space primordial CMB fields can lead to off diagonal correlations between the harmonic space fields, where $l\neq l'$ terms are also non-zero.
\par 
In the case of the specific distortion we consider in this paper, the temperature and polarization leakage is treated as a small spin-2 correction to the complex Stokes parameters of the form

\begin{equation}\label{eqn:Stokes Parameter Perturbation}
    {}_{\pm}P(\hat{\mathbf{n}}) + {}_{\pm}\delta P(\hat{\mathbf{n}}) = (\Tilde{Q}\pm i\Tilde{U})(\hat{\mathbf{n}}) + (\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})\Tilde{T}(\hat{\mathbf{n}})\;.
\end{equation}
In this work $\gamma^{Q}$ and $\gamma^{U}$ are  the $Q$ and $U$ like components of the spin-2 temperature to polarization leakage field respectively and are constructed from the product of the gain systematic and the scan. In a realistic case our data model is such that
\begin{equation}
    d = X*B + G\cdot (T*b) + N\;
\end{equation}
Here $X$ represents the polarization maps, $*$ represents a convolution with the beams $B$ for the polarization beam and $b$ for the temperature beam, $G$ represents the temperature to polarization leakage fields, the $\cdot$ represents a multiplication, and N represents the noise.
A perturbation to the stokes parameters will propagate through the $E$ and $B$ mode polarisation decomposition giving additional corrections to the $E$ and $B$ mode harmonic space fields. Details of how these perturbations propogate can be found in appendix \ref{app:QE appendix}. The corrections to $E$ are
\begin{equation}
    \label{eqn:delta elm gamma E}
    \delta E_{lm} = \sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{E}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{equation}
for $l+L+l_{2} =$ even, and
\begin{equation}
    \label{eqn:delta elm gamma B}
    \delta E_{lm} =
    -i\sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{B}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{equation}
for $l+L+l_{2} =$ odd. The corrections to $B$ are
\begin{eqnarray}
    \label{eqn:delta blm gamma E}
    \delta B_{lm} =
    i\sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{E}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{eqnarray}
for $l+L+l_{2} =$ odd, and
\begin{eqnarray}
    \label{eqn:delta blm gamma B}
    \delta B_{lm} = \sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{B}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,\;,
\end{eqnarray}
for $l+L+l_{2} =$ even.
Here $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ are are related to $\gamma^{Q}(\hat{\mathbf{n}})$ and $\gamma^{U}(\hat{\mathbf{n}})$ through a spin-2 spherical harmonic transformation in analogy to the transformation between the $E_{lm}$ and $B_{lm}$ fields and the $Q(\hat{\mathbf{n}})$ and $U(\hat{\mathbf{n}})$ fields. The $\xi^{LM}_{lml'm'}$ and $\mathcal{H}^{L}_{ll'}$ are Wigner-3j geometric terms that encode the coupling between modes inherent in the introduction of such additional anisotropic corrections to the harmonic space fields. The exact forms of the geometric terms are found in appendix \ref{app:QE appendix}. 
\par 
Such corrections to the $E_{lm}$ and $B_{lm}$ manifest themselves in the off diagonal auto- and cross-correlations between the harmonic space fields. The anisotropic systematics introduce a degree of statistical anisotropy that lead to correlations in the off diagonal. One can see off diagonal correlations if, for example, one takes the cross correlations between the $T_{lm}$ and $B_{lm}$ fields. Assuming no primordial $B$-mode polarisation the result is
\begin{equation}\label{eqn:deltaB T cross gamma B}
    \left\langle B_{lm}T^{*}_{l'm'}\right\rangle = \sum_{LM}\gamma_{LM}^{B}\tilde{C}^{TT}_{l'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'} \;,
\end{equation}
for $l+L+l' =$ even, and 
\begin{equation}\label{eqn:deltaB T cross gamma E}
    \left\langle B_{lm}T^{*}_{l'm'}\right\rangle = i\sum_{LM}\gamma_{LM}^{E}\tilde{C}^{TT}_{l'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'} \;,
\end{equation}
for $l+L+l' =$ odd. Here, we discard any terms that are higher than first order in $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$, as these are expected to be small. Tilde symbols are used denote that a given $C_{l}$ is the power spectrum for a primordial CMB field. As the primordial, on diagonal contributions to $\left\langle B_{lm}T^{*}_{l'm'}\right\rangle$ are zero, both \eqref{eqn:deltaB T cross gamma B} and \eqref{eqn:deltaB T cross gamma E} contain only on- and off-diagonal anisotropic contributions from the temperature to polarization leakage distortion.

\subsection{Estimating the distortion} 
It is possible to use the presence of additional statistical anisotropy and off diagonal terms in the correlations between the harmonic space fields in order to estimate the distortion fields $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ This is done by inverting \eqref{eqn:deltaB T cross gamma B} and \eqref{eqn:deltaB T cross gamma E}. For simplicity we collect the terms in \eqref{eqn:deltaB T cross gamma B} into $J^{LM,',XX'}_{ll'}$ and the terms in \eqref{eqn:deltaB T cross gamma E} into $K^{LM,',XX'}_{ll'}$ where,
\begin{equation}J^{LM,',XX'}_{ll'}\equiv\gamma^{B}_{LM}Z^{XX'}_{ll'}\;,
\end{equation}
and 
\begin{equation} 
K^{LM,',XX'}_{ll'}\equiv\gamma^{E}_{LM}\zeta^{XX'}_{ll'}\;.
\end{equation}
The definitions of $Z^{XX'}_{ll'}$ and $\zeta^{XX'}_{ll'}$ for a given choice of $XX'$ can be seen in table \ref{tab:Z values}. 
\begin{table}[!htp]
\caption{Table of $Z^{L,\,A}_{ll'}$ and $\zeta^{L,\,A}_{ll'}$ along with the with the parity for which the terms are required to be non-zero.\label{tab:Z values}}
    \centering
    \begin{tabular}{c|cc|cc|}
     $XX'$ & $Z^{A}_{ll'}$ & parity requirements & $\zeta^{A}_{ll'}$ & parity requirements\\
     &&&&\\
     \hline
     \hline
     &&&&\\
     $BT$ & $C^{TT}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ even & $-iC^{TT}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ odd\\ 
     &&&&\\
     $TB$ & $C^{TT}_{l}H^{L}_{ll'}$& $l+l'+ L =$ even & $iC^{TT}_{l}H^{L}_{ll'}$ & $l+l'+ L =$ odd \\
     &&&&\\
     $BE$ & $C^{TE}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ even & $-iC^{TE}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ odd \\
     &&&&\\
     $EB$ & $C^{TE}_{l}H^{L}_{ll'}$ & $l+l'+ L =$ even & $iC^{TE}_{l}H^{L}_{ll'}$ & $l+l'+L =$ odd\\
     &&&&\\
     $EE$ & $i(C^{TE}_{l'}-C^{TE}_{l})$ & $l+l'+ L =$ odd& $C^{TE}_{l} + C^{TE}_{l'}$  & $l+l'+ L =$ even\\
\end{tabular}
\end{table}
It is possible to write estimators for  $J^{LM,',XX'}_{ll'}$ and $K^{LM,',XX'}_{ll'}$ in terms of the observed CMB fields, the exact detail of how this is done is seen in appendix \ref{app:QE appendix 2}. It is then merely a matter of dividing these anisotropic terms by any unwanted terms in order to give $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$. That is, for a given set of multipoles $ll'$ and choice of fields $XX'$ (shortened to $A$),
\begin{eqnarray}
    (\widehat{\gamma}^{B}_{LM})^{A}_{ll'} =&&\, \frac{\widehat{J}^{LM,\,A}_{ll'}}{F^{L,\,A}_{ll'}}\;,\label{eqn:gamBhat}\\
    (\widehat{\gamma}^{E}_{LM})^{A}_{ll'} =&&\, \frac{\widehat{K}^{LM,\,A}_{ll'}}{\mathcal{F}^{L,\,A}_{ll'}}\;.\label{eqn:gamEhat}
\end{eqnarray}
Here, the hats on $\widehat{J}^{LM,\,A}_{ll'}$ and $\widehat{K}^{LM,\,A}_{ll'}$ indicate that they are the estimators. Moreover, the terms that are divided through are defined as  $F^{L,\,A}_{ll'}\equiv Z^{A}_{ll'}W_{l}W_{l'}$ and $\mathcal{F}^{L,\,A}_{ll'}\equiv \zeta^{A}_{ll'}W_{l}W_{l'}$ and contain the beam window function $W_{l}$. Inverse variance weighting can be used to move from an estimate for a given multipole pair and choice of $A$ to a full averaged estimate. This inverse variance weighted average takes the form 
\begin{equation}\label{eqn:gamma E estimator}
    \widehat{\gamma}^{E}_{LM} = \mathcal{N}^{E}_{L}\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}\mathcal{F}^{L,A'}_{ll'}\widehat{K}^{LM,\,A}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\;,
\end{equation}
where and $\mathcal{C}^{ll'}_{AA'}$ is the covariance matrix for the covariance of $\widehat{K}^{LM,\,A}_{ll'}$ and 
\begin{equation}
    G^{L}_{ll'} = \frac{(2l+1)(2l'+1)}{4\pi}\;.
\end{equation}
Here, $\mathcal{N}^{E}_{L}$ represents the reconstruction noise for the estimator and is included due to the inverse variance weighting. It is calculated as follows:
\begin{equation}\label{eqn:reconstruction noise for gamma E}
    \mathcal{N}^{E}_{L} = \left(\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}\mathcal{F}^{L,\,A}_{ll'}\mathcal{F}^{L,\,A'}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\right)^{-1}\;.
\end{equation}
The full estimator for $\gamma^{B}_{LM}$ has the similar form 
\begin{equation}\label{eqn:gamma B estimator}
    \widehat{\gamma}^{B}_{LM} = \mathcal{N}^{B}_{L}\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}F^{L,A'}_{ll'}\widehat{J}^{LM,\,A}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\;,
\end{equation}
and
\begin{equation}\label{eqn:reconstruction noise for gamma B}
    \mathcal{N}^{B}_{L} = \left(\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}F^{L,\,A}_{ll'}F^{L,\,A'}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\right)^{-1}\;.
\end{equation}

The summation over $l$ is limted to $l\leq l'$ to avoid over counting as under the exchange of indices $l\leftrightarrow l'$ the exchange of fields $XX' \leftrightarrow X'X$ occurs. One does not need such measures if the estimator is limited to using either $XX'$ or $X'X$. However, this is less efficient in harmonic space than using both $XX'$ and $X'X$ with the limited $l$ range.

\subsection{Efficient estimators}
\par
Due to the presence of the Wigner-3j symbol containing geometric terms these estimators are very computationally demanding, scaling as $\sim l^{4}$.  It is possible to write the estimators of specific combinations of modes, for example $TB$ only. This is beneficial as some combinations of modes perform better than others, often performing so well that using more than one combination of modes is unnecessary. Moreover, using fewer mode combinations requires less computing time. However, to further reduce computing time it is also necessary to rewrite these estimators in a way that avoids calculating a large number of Wigner-3j symbols. As these estimators involve a convolution in harmonic space they can be written as simple products of the real space fields, thus avoiding computing any Wigner-3j symbols. We begin by writing the estimators that only use the $TB$ modes,
\begin{equation}
    \widehat{\gamma}^{B}_{LM} = 
    \mathcal{N}^{B}_{L}\sum_{l l'mm'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'}\frac{B_{lm}T^{*}_{l'm'}}{C^{BB,\,\rm map}_{l}C^{TT,\,\rm map}_{l'}}\tilde{C}^{TT}_{l'}W_{l}W_{l'}\;,
\end{equation}
where $l+l'+L= {\rm even}$ and
\begin{equation}
    \widehat{\gamma}^{E}_{LM} = -i\mathcal{N}^{E}_{L}\sum_{l l'mm'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'}\frac{B_{lm}T^{*}_{l'm'}}{C^{BB,\,\rm map}_{l}C^{TT,\,\rm map}_{l'}}\tilde{C}^{TT}_{l'}W_{l}W_{l'}\;,
\end{equation}
where $l + l' + L = {\rm odd}$. Note that we have not limited sum over $l$ to $l\leq l'$. Limiting the range of the sum is unnecessary in the case of the efficient estimators as this sum is never explicitly carried out.
The reconstruction noises for these TB only estimators are
\begin{equation}\label{eqn:TB noise B}
    \mathcal{N}^{B}_{L} = \sum_{l'\geq l}(1+\delta_{ll'})^{-1}G^{L}_{ll'}\left[\frac{\left|F^{L,BT}_{ll'}\right|^{2}}{C^{BB,\,\rm map}_{l}C^{TT\,\rm map}_{l'}} + \frac{\left|F^{L,TB}_{ll'}\right|^{2}}{C^{TT,\,\rm map}_{l}C^{BB\,\rm map}_{l'}}\right]\;,
\end{equation}
and,
\begin{equation}
    \mathcal{N}^{E}_{L}= \sum_{l'\geq l}(1+\delta_{ll'})^{-1}G^{L}_{ll'}\left[\frac{\left|\mathcal{F}^{L,BT}_{ll'}\right|^{2}}{C^{BB,\,\rm map}_{l}C^{TT\,\rm map}_{l'}} + \frac{\left|\mathcal{F}^{L,TB}_{ll'}\right|^{2}}{C^{TT,\,\rm map}_{l}C^{BB\,\rm map}_{l'}}\right]\;.
\end{equation}
We do not write reconstruction noise in a more efficient form so the limit $l\leq l'$ still applies when calculating $\mathcal{N}^{B}_{L}$ and $\mathcal{N}^{E}_{L}$. In principle $C^{\rm map}_{l} = W^{2}_{l}\tilde{C}_{l} + C^{\,\rm noise}_{l}$, where $C^{\,\rm noise}_{l}$ is the noise power spectrum, and $W_{l}$ is the beam window function given by $W_{l} \approx \exp(-l^{2}\sigma_{b}^{2}/2)$ with $\sigma_{B} = \Theta_{\rm FWHM}/\sqrt{8\ln2}$ \cite{Kamionkowski1997a}. However, in practice $C^{\rm map}_{l}$ must be directly estimated from the polarization maps as their values are effected significantly by the presence of the temperature to polarization leakage.  $C^{\rm map}_{l} = \tilde{C}_{l} + C^{\,\rm noise}_{l}$. The geometric kernel terms $\xi^{LM}_{lml'm'}$ and $\mathcal{H}^{L}_{ll'}$ can be written as real space integrals of spin weighted spherical harmonics. When this is done, taking into account the difference in parity between the two estimators one arrives at the efficient estimators,
\begin{eqnarray}
    \widehat{\gamma}^{B}_{LM} =&&\,\frac{\mathcal{N}^{B}_{L}}{2}\int d\hat{\mathbf{n}}\big[{}_{-2}Y_{LM}(\hat{\mathbf{n}}){}_{-2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\nonumber\\ 
    &&\,+ {}_{+2}Y_{LM}(\hat{\mathbf{n}}){}_{+2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\big]\;,
\end{eqnarray}
and 
\begin{eqnarray}
    \widehat{\gamma}^{E}_{LM} =&&\,\frac{-i\mathcal{N}^{E}_{L}}{2}\int d\hat{\mathbf{n}}\big[{}_{-2}Y_{LM}(\hat{\mathbf{n}}){}_{-2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\nonumber\\ 
    &&\,- {}_{+2}Y_{LM}(\hat{\mathbf{n}}){}_{+2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\big]\;.
\end{eqnarray}
Here the real space fields are written as transforms of the harmonic space $E_{lm}$ and $B_{lm}$ terms in the following forms:
\begin{eqnarray}
    {}_{s}A_{X}(\hat{\mathbf{n}}) =&&\, \sum_{lm}\frac{1}{C^{XX}_{l}}X_{lm}{}_{s}Y_{lm}(\hat{\mathbf{n}})\;,\\
    {}_{s}A^{XY}_{X'}(\hat{\mathbf{n}}) =&&\, \sum_{lm}\frac{\tilde{C}_{l}^{XY}}{C^{X'X'}_{l}}X'_{lm}{}_{s}Y_{lm}(\hat{\mathbf{n}})\;,
\end{eqnarray}


==> sections/old_files/recap.tex <==
\section{Distortion Fields}
\label{sec:recap}
In the ideal scenario the true CMB polarisation signal would be isolated and easily measurable. However in reality it is subject to a plethora of contaminants. A number of these contaminants can be characterised by their spin dependence and as such readily written in to a set of distortion fields.


The work of \cite{2010PhRvD..81f3512Y} and \cite{2003PhRvD..67d3004H} describe the effects of various cosmological signals and systematic effects on the measured polarisation at map level through 11 distortion fields as
\begin{eqnarray}
    {}_{\pm}\delta P(\hat{\mathbf{n}}) &&= [a \pm i 2\omega](\hat{\mathbf{n}}){}_{\pm}P(\hat{\mathbf{n}}) + [f_{1} \pm if_{2}](\hat{\mathbf{n}}){}_{\mp}P(\hat{\mathbf{n}}) + [\gamma_{1} \pm i\gamma_{2}](\hat{\mathbf{n}})\tilde{T}(\hat{\mathbf{n}})
    \nonumber\\
    &&+\sigma \mathbf{{}_{1}p}(\hat{\mathbf{n}}) \cdot {}_{\mp}\nabla {}_{\pm}P(\hat{\mathbf{n}};\sigma) + \sigma [d_{1} \pm id_{2}](\hat{\mathbf{n}}) [\partial_{1} \pm i\partial_{2}]\tilde{T}(\hat{\mathbf{n}};\sigma) +\sigma^{2}q(\hat{\mathbf{n}})[\partial_{1} \pm i\partial_{2}]^{2}\tilde{T}(\hat{\mathbf{n}};\sigma) + ...
    \label{eqn:Distortion Fields}
\end{eqnarray}
where ${}_{\pm}P(\hat{\mathbf{n}}) = \tilde{Q} \pm \tilde{U}$ is the spin-2 polarisation and ${}_{\pm}\delta P(\hat{\mathbf{n}})$ corresponds to some correction to the polarisation field. It is worth noting here that the form of these distortion fields will be highly dependent on the scanning strategy and as such a realistic scan should be employed when considering drawing conclusions. We look at this in detail in section \ref{sec:Realistic Scan}.


Equation \ref{eqn:Distortion Fields} has been constructed such that the top line corresponds to mixing between polarisation and temperature in a known direction on the sky. While the bottom line considers mixing in a local region with some directional dependence such that they leak the derivative of the CMB fields, e.g. pointing or lensing. The length scale $\sigma$ corresponding to the width of a Gaussian beam that is smoothing the CMB fields. The second line quantities are sourced by a simple first order Taylor expansion of the CMB fields around $\hat{\mathbf{n}}$, however a number of first order contaminants have been neglected in this equation which we shall explore in section \ref{sec:Additional Terms}.


Since ${}_{\pm}P$ is a spin $\pm2$ field the distortions to this must be spin $\pm2$ also, this necessitates that $a(\hat{\mathbf{n}})$ and $\omega(\hat{\mathbf{n}})$ are scalar fields describing an amplitude scaling and a polarisation plane rotation respectively, $[f_{1} \pm if_{2}](\hat{\mathbf{n}})$ is a spin $\pm 4$ field which couples the conjugate polarisation fields, $[\gamma_{1} \pm i\gamma_{2}](\hat{\mathbf{n}})$ is a spin $\pm2$ field that couples the temperature to polarisation directly. $\mathbf{{}_{1}p}(\hat{\mathbf{n}}) = {}_{1}[p_{1} \pm ip_{2}](\hat{\mathbf{n}})$ is a spin $\pm1$ deflection field that describes direction changes of the photons, $[d_{1} \pm id_{2}](\hat{\mathbf{n}})$ is a spin $\pm1$ field and $q(\hat{\mathbf{n}})$ is a scalar field that couple the first and second derivatives of the temperature field to the polarisation respectively. Since there are no known processes that cause T to P conversion along the line of sight each of the T containing terms can be attributed to some systematic.



Each of the terms in equation \ref{eqn:Distortion Fields} may be attributed to some cosmological signal or systematic. We will not provide an exhaustive list here but will pick out some important terms to explore. It is indicated in \citep{2010PhRvD..81f3512Y} that the $(\gamma_{1}\pm i\gamma_{2})(\hat{\mathbf{n}})$ field poses the largest B-mode contaminant. As such we have chosen to concentrate on this field which hereafter we relabel $(\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})$ in analogy with the stokes parameters. The source of this particular field which leaks temperature to polarisation can be attributed to a differential gain systematic. Indeed, the distortion fields we focus on in this work are the differential gain that induce temperature to polarization leakage. While we choose a specific distortion, we do this with the aim of demonstrating cleaning and reconstruction techniques that could be more generally applicable to the full list of distortions seen in equation \eqref{eqn:Distortion Fields}.


\subsection{Additional Terms}
\label{sec:Additional Terms}
Some additional terms that contribute to the distortion field, that were neglected in equation \ref{eqn:Distortion Fields} sourced from \citep{2010PhRvD..81f3512Y} include
\begin{eqnarray}
\label{eqn:Additional Distortion Terms}
    {}_{\pm}\delta P^{\text{New}}(\hat{\mathbf{n}}) &&= \sigma \mathbf{{}_{-1}p}(\hat{\mathbf{n}}) \cdot {}_{\pm}\nabla {}_{\pm}P(\hat{\mathbf{n}};\sigma) + \sigma \mathbf{{}_{3}p}(\hat{\mathbf{n}}) \cdot {}_{\pm}\nabla {}_{\mp}P(\hat{\mathbf{n}};\sigma) + \sigma \mathbf{{}_{5}p}(\hat{\mathbf{n}}) \cdot {}_{\mp}\nabla {}_{\mp}P(\hat{\mathbf{n}};\sigma)
    \nonumber\\
    &&+ \sigma \mathbf{{}_{3}d}(\hat{\mathbf{n}}) [\partial_{1} \mp i\partial_{2}]\tilde{T}(\hat{\mathbf{n}};\sigma) + \sigma^{2} \mathbf{{}_{4}q}(\hat{\mathbf{n}})[\partial_{1} \mp i\partial_{2}]^{2}\tilde{T}(\hat{\mathbf{n}};\sigma).
\end{eqnarray}
These additional terms correspond to additional leading order terms in the Taylor expansion that describe the directional dependent contaminants of equation \ref{eqn:Distortion Fields}. It is important not to neglect these terms as there are a number of systematics that would result in these distortion fields being non-zero. We point out in particular that a differential pointing systematic, which would contribute to the terms containing the $[d_{1} \pm id_{2}](\hat{\mathbf{n}})$ and $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$ field in equation \ref{eqn:Distortion Fields}, also contributes to a number of other terms in equation \ref{eqn:Additional Distortion Terms}. This includes additional coupling of the conjugate of the derivative of the Temperature field with the Polarisation through the spin-3 $\mathbf{{}_{3}d}(\hat{\mathbf{n}})$ field, which through examining figure \ref{fig:Distortion Fields} it is clear contributes a systematic of similar level to the spin-1 contribution and as such should not be neglected. In addition the differential pointing will also contribute to the terms containing the fields $\mathbf{{}_{-1}p}(\hat{\mathbf{n}})$, $\mathbf{{}_{5}p(\hat{\mathbf{n}})}$, and $\mathbf{{}_{3}p(\hat{\mathbf{n}})}$ which induce polarisation mixing as detailed in \cite{2020arXiv200800011M}. With the unprecedented sensitivity levels planned for future CMB missions it is more important than ever to understand the systematics present, and not neglect any of the terms that could bias measurements.


\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/DistortionFields.pdf}
    \caption{The left column shows maps of the spin-2 $(\gamma_{1}+i\gamma_{2})(\hat{\mathbf{n}})$ distortion field sourced by a 1\% differential gain systematic which causes a T leakage into the polarisation. The second and third columns show the spin-1 $({}_{1}d_{1}+i{}_{1}d_{2})(\hat{\mathbf{n}})$ and spin-3 $({}_{3}d_{1}+i{}_{3}d_{2})(\hat{\mathbf{n}})$ distortion fields sourced by a $0.1'$ differential pointing systematic which causes a leakage of the derivative of the temperature into the polarisation. These fields have been calculated analytically using the product of the appropriate spin scan field and the systematic as explained in section \ref{sec:Differential Gain} with further information available in \cite{2020arXiv200800011M}.  There is clearly significant difference between the distortion fields sourced by different systematics, though the structure of the scan is visible in all. This demonstrates that taking into account the scan strategy for such systematics is pivotal to fully understand the viability of methods to reconstruct systematics. Note that the spin 1 and 3 fields of the middle and right panels are of a similar magnitude suggesting each will contribute a comparable level of differential pointing systematic which is not negligible.}
    \label{fig:Distortion Fields}    
\end{figure}


%\subsection{Issues for Lensing Estimators}
%\AR{We can skip these details for this paper. We can have a brief discussion on this when we present perspectives. This doesnt fit in to other details we discuss in this paper.}
%When travelling from the surface of last scattering to us the CMB photons are subjected to deflections by the intervening matter. This effect known as weak gravitational lensing causes a redistribution of the CMB photons and may be written as \cite{1998PhRvD..58b3003Z,2003PhRvD..68h3002H,2005PhRvD..71l3527C}
%\begin{eqnarray}
%    {}_{\pm}\delta P(\hat{\mathbf{n}}) &&= {}_{\pm}P(\hat{\mathbf{n}} + \nabla \Phi + \nabla \times \Omega)\nonumber
%    \\
%    &&= \nabla \Phi \cdot \nabla {}_{\pm}P(\hat{\mathbf{n}}) + \nabla \times \Omega \cdot \nabla {}_{\pm}P(\hat{\mathbf{n}}) + ...
%\end{eqnarray}
%where the second line has been written using the Taylor expansion about $\hat{\mathbf{n}}$. The deflection field $\nabla \Phi$ is sourced by linear order density perturbations in the intervening matter where $\Phi$ is the projected gravitational potential along the line of sight. While the $\nabla \times \Omega$ deflection field would be sourced by higher order scalar gravitational potentials (e.g. deflection by multiple lenses along the line of sight) or by exotic non-$\Lambda$CDM matter (e.g. topological defects). The curl part is usually much smaller than the grad and is generally treated as vanishingly small. However there is a further source that can contribute to both the grad and curl components, a contamination from systematics.



%The deflection field $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$ included in equation \ref{eqn:Distortion Fields} is attributed to the effect of lensing when considered in \citep{2010PhRvD..81f3512Y}. The gradient term $\nabla \Phi$ contributes to the $p_2(\hat{\mathbf{n}})$ deflection field and the curl term is contained in $p_1(\hat{\mathbf{n}})$ deflection field. However fields of this form can also be sourced by a number of systematics, which as such could cause a bias when attempting lensing reconstruction. The work of \cite{2005PhRvD..71l3527C} for instance advocates using the presence of a curl component as systematic diagnostic.


%We point out here in particular that, as shown in \cite{2020arXiv200800011M}, the form of the differential pointing systematic means it could mimic both the grad and curl parts of lensing. We already noted that a T-P coupling is generated by the differential pointing systematic, however the differential pointing will also contribute as a deflection field acting on the polarisation directly and as such will contaminate the lensing contribution to the deflection field $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$. This is an important observation to make as consequently the presence of a differential pointing systematic could interfere with the QE used to reconstruct CMB lensing and vice versa. Furthermore this excess signal from differential pointing could in principle cause an overestimation of the lensing amplitude parameter $A_{lens}$ \cite{2008PhRvD..77l3531C}. As the differential pointing contributes to other terms in equations \ref{eqn:Distortion Fields} and \ref{eqn:Additional Distortion Terms} that the CMB lensing signal does not, it could in principle be possible to combine the QE for these fields along with prior information of the scan strategy to disentangle the systematic from the lensing signal. We leave this to further work to explore in detail.





==> sections/old_files/reconstructionold.tex <==
\section{Optimal filtering for cleaning and reconstruction}

\subsection{Map and power spectrum reconstruction with map filtering}
The efficient form of the quadratic estimators are applied to the CMB Temperature map, $T(\uvec{n})$, and polarization maps, $Q(\uvec{n})$ and $U(\uvec{n})$ produced by the simulations described in \ref{sub:Simulation}. The resulting reconstructed harmonic space temperature to polarization leakage fields, $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$, must be filtered so that modes that are saturated by reconstruction noise are down-weighted in comparison to high signal to noise ratio (SNR) modes. We define SNR at each multipole, $L$, as 
\begin{equation}
    \text{SNR}_{L} = \frac{\widehat{C}^{\gamma^{\chi\chi}}_{L}-\mathcal{N}^{\chi}_{L}}{\sqrt{\frac{2}{2L+1}}\mathcal{N}^{\chi}_{L}}\;,
\end{equation}
where $\widehat{C}^{\gamma^{\chi\chi}}_{L}$ is the estimator for the power-spectum of either $\gamma^{E}_{LM}$ or $\gamma^{B}_{LM}$, defined as 
\begin{equation}
    \widehat{C}^{\gamma^{\chi\chi}}_{L} \equiv \sum_{M=-L}^{L}\frac{\left|\widehat{\gamma}^{\chi}_{LM}\right|^{2}}{2L+1}
\end{equation}
Our filter is constructed so that
\begin{equation}
F^{\chi\chi}_{L} = \begin{cases}
    0, & \text{if SNR}_{L} \leq 1\\
    A\exp\left(-\left[\frac{\widehat{C}^{\gamma^{\chi\chi}}_{L}}{\widehat{C}^{\gamma^{\chi\chi}}_{L}-\mathcal{N}^{\chi}_{L}}\right]^{2}\right),&\text{if SNR}_{L} > 1\\
\end{cases}\;.
\label{eqn:filter}
\end{equation}
The filter is normalized by $A$ so that the maximum value the filter will take is $F^{\chi\chi}_{L} = 1$. These filters are applied in harmonic space to the $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ fields. These fields are transformed to the real space, $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$, fields.
\par 
In figure \ref{fig:map comparisons} we compare the resulting filtered, reconstructed temperature to polarization leakage maps, $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$, to the actual leakage maps calculated directly from the input differential gain and prior knowledge of the scan, and to the actual leakage fields with only information up the $L_{\rm max}$ of the reconstructed fields.
\par 
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_hybrid_real_multiplot_map_Lmax_1000_lmax_3000.pdf}
    \caption{A comparison of the true systematic maps (left) and the systematic maps reconstructed up to $L=1000$ using an efficient quadratic estimator (right). Also presented here is the true systematic map with multipole information of $L>1000$ removed (center). The noise and beam for the simulated maps are chosen to emulate the proposed \textit{LiteBIRD} experiment \cite{Hazumi2019}.}
    \label{fig:map comparisons}    
\end{figure}
The features of the input leakage maps are correctly reconstructed. When comparing the reconstructed maps to the input maps only in the range the reconstruction was performed over we see that the amplitudes of the reconstructed maps match the input maps. The amplitude of the full input maps is larger than the reconstructed due to the extra power coming from the modes above $L_{\rm max}$.
\par 
The efficacy of the reconstruction and the importance of filtering is better seen in a comparison between the power spectra of the true and \emph{unfiltered} reconstructed systematic maps; such a comparison can be seen in figure \ref{fig:ps comparisons}. 
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_hybrid_real_gamma_EandB_powspec_Lmax_1000_lmax_3000_iter_0.pdf}
    \caption{A comparison of the true $C^{\gamma^{EE}}_{L}$ and $C^{\gamma^{BB}}_{L}$ power spectra (blue dots) and the $\widehat{C}^{\gamma^{E}}_{L}$ and $\widehat{C}^{\gamma^{B}}_{L}$ quadratic estimator reconstructed power spectra (orange dots) in the range $2\leq L\leq1000$ with no filtereing applied. The noise and beam for the simulated maps are chosen to emulate the proposed \textit{LiteBIRD} experiment \cite{Hazumi2019}. It can be seen that the reconstruction noise (red) becomes dominant at $L\sim50$ for both sets of power spectra. \NM{MLB Comment - Need to make very clear that although the reconstruction noise is dependent on the signal, this is not a problem because you measure the reconstruction noise (in addition to the "signal + noise" power directly from the map. (This currently doesn't come across at all in either the main text or the caption.) (Comment applies to this figure, and the associated discussion in the text in section D.)}}
    \label{fig:ps comparisons}    
\end{figure}
Note that in the $L$ range below $L=50$ the power spectra of the input maps and unfiltered, reconstructed maps match. However, the reconstruction noise becomes dominant at $L\sim 50$ and it is impossible to effectively reconstruct the systematic maps at these higher multipoles. That is, at the smaller scales corresponding to these higher multipoles the reconstructed maps will be dominated by the reconstruction noise. These are the modes that must be down-weighted through filtering in order to give a leakage map that is not heavily biased by the reconstruction noise.

\subsection{Reconstructing different levels of differential gain}

We run the simulation described in section \ref{sub:Simulation} for $\delta g_{1} = \delta g_{2} = $ 0.01, 0.001, and 0.0001. We show the $\widehat{C}^{\gamma^{EE}}_{L}$ and $\widehat{C}^{\gamma^{BB}}_{L}$ power spectra recovered from the unfiltered, reconstructed maps, the reconstruction noise, and $C^{\gamma^{EE}}_{L}$ and $C^{\gamma^{BB}}_{L}$ from the input maps for all three gain levels in figure \ref{fig:gain levels}.
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/diff_gain_comp_nonoise_gamma_EandB_powspec_Lmax_100_lmax_500.pdf}
    \caption{Reconstructed $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$ spectra and reconstruction noise for a 1\% (orange) , 0.1\% (red), and 0.01\% (magenta) differential gain. The input $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$ spectra are also displayed in blue, green and black for the 1\%, 0.1\% and 0.01\% differential gain respectively.}
    \label{fig:gain levels}    
\end{figure}
\par 
For all three levels of differential gain the quality of reconstruction appears to be similar, with a similar maximum $L$ at which the reconstruction is not dominated by noise. The amplitude of the reconstruction noise appears to be proportional to the level of systematic included in the scan. This is to be expected as the variance of the observed CMB power spectra $C_{l}^{TT}$ and $C_{l}^{BB}$ feeds directly into the covariance matrix for the quadratic estimator. Therefore, a systematic which increases the variance of these spectra will increase the covariance for the quadratic estimator and therefore increase the reconstruction noise for $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$. 
\par 
We also performed this study keeping $\delta g_{1}$ and $\delta g_{2}$ fixed but allowing $w^{-1/2}_p$ to take the values in the range $w^{-1/2}_p=0\mu\text{K-arcmin}$ to $w^{-1/2}_p=5\mu\text{K-arcmin}$. Changing the pixel noise resulted in different levels of reconstruction noise. However, the change in reconstruction noise is small, and has only a small effect on the $L$ at which the reconstruction noise becomes dominant. The $L$ at which the noise saturates the reconstruction is only a factor of $\sim2$ less for $w^{-1/2}_{p} = 5\mu\text{K-arcmin}$ than for $=w^{-1/2}_{p}\mu\text{K-arcmin}$. The input differential gain has a much more profound effect on amplitude of the reconstruction noise.
\par
The quadratic estimator technique can be used as an excellent tool to diagnose temperature to polarization leakage in CMB maps without prior knowledge of the instrument or scan because it is possible to reconstruct even very low levels of temperature to polarization leakage effectively. For all three levels of differential gain there is a maximum $L$ beyond which the reconstruction noise dominates. However, below this multipole it is possible to precisely reconstruct the temperature to polarization leakage systematic.

==> sections/primordial_B.tex <==
\section{Implications for primordial B-modes}
\label{sec:Primordial B-modes}
\subsection{Removing leaked B-mode power and measuring primordial B-mode power spectrum}
A temperature to polarization leakage would introduce a large contaminant in the search for primordial tensor perturbations. Therefore, it is necessary to mitigate such a systematic. Often to do this prior knowledge of the scanning strategy and the instrument with which the CMB measurements are taken is necessary and complicated modeling techniques are utilized \cite[e.g.][]{2015ApJ...814..110B,2016A&A...594A...3P}. However, if it is possible to blindly reconstruct the systematic from the map level data alone it may also be possible to self clean the maps themselves and recover a systematic cleaned $B$-mode power spectrum.
\par 
We apply our quadratic estimator to the maps produced by the simulations described in section \ref{sub:Simulation} in order to demonstrate the that it is possible to self clean maps using the reconstructed systematic. The filter in equation \eqref{eqn:filter} is then applied to the harmonic space leakage maps. We then solve equation \eqref{eqn:Stokes Parameter Perturbation} for the primordial $\tilde{Q}$ and $\tilde{U}$, using our reconstructed and filtered $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$, in order to recover the primordial $\tilde{Q}(\hat{\mathbf{n}})$ and $\tilde{U}(\hat{\mathbf{n}})$. As the reconstruction noise is proportional to the level of temperature to polarization leakage remaining the in the CMB polarization maps we are able to iteratively clean the polarization maps. That is, the process of reconstructing $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$ and inverting equation \eqref{eqn:Stokes Parameter Perturbation} to recover $\tilde{Q}(\hat{\mathbf{n}})$ and $\tilde{U}(\hat{\mathbf{n}})$ is repeated for multiple iterations. It is possible that some modes which were previously noise saturated will become signal dominated after each iteration, and therefore with each iteration more cleaning is possible.
\par 
It is difficult to see, at map level, the effect that this cleaning has had, and how well the primordial polarisation has been recovered. However, at power spectrum level the effect that this cleaning has on the polarisation is clearer. In Figure.~\ref{fig:cleaned BB} we show the $B$-mode power recovered from the scan maps before cleaning, and from a map where no systematic was injected initially. We then compare these systematic free and systematic saturated $B$-mode spectra to the cleaned $B$-mode after 0, 1, 2 and 3 iterations of the cleaning process. Even with the very simple cleaning process used there is a large suppression of the temperature to polarisation leakage systematic. Self cleaning the maps suppresses the systematic effect by over an order of magnitude at the $\ell=80$ peak of the $B$-mode power spectrum, providing near perfect cleaning at this mode after only two iterations of the cleaning.
\par 
Increasing the number of iterations improves the cleaning up until two iterations. In Figure.~\ref{fig:cleaned BB} we see that increasing the number of iterations to three actually introduces further contamination. This contamination come from the effects of beam smearing and the Gaussian white noise on the variance of the reconstruction of the systematics maps. There is an optimum number of iterations for this self cleaning. However, at this optimum number of iterations Figure.~\ref{fig:cleaned BB} suggests it may be possible to recover important parts of the primordial $B$-mode power spectrum.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_hybrid_real_cleaned_BB_comparison_Lmax1000_lmax3000_iter_2.pdf}
    \caption{The $B$-mode power spectrum for the polarization maps simulated with a 1\% differential gain (black) and  no differential gain (blue), and the power spectrum of the cleaned maps for 0 iterations of cleaning (brown), 1 iteration of cleaning (purple), 2 iterations of cleaning (red), and three iterations of cleaning (orange). Also shown as a green band is the primordial $B$-mode power spectrum for a range of possible values of $r$ from $r=10^{-2}$ to $r=10^{-3}$. The lensing spectrum is also shown (magenta line).}
    \label{fig:cleaned BB}
\end{figure}




\subsection{Tensor to scalar ratio}
In order to constrain the extent to which cleaning matters it is worth examining it within the context of the tensor to scalar ratio. We use the prescription presented in appendix B of \citep{2010PhRvD..81f3512Y} for this where the uncertainty in the tensor to scalar ratio $\Delta r$ may be compared between the cases where the cleaning has and has not been applied. We choose the best cleaning scenario, where two iterations of cleaning have been carried out. We integrate over B-modes in the $2\leq\ell\leq200$ range, which is appropriate for an experiment with a large beam like \emph{LiteBIRD}. The ratio between the not cleaned and cleaned case $\Delta r_{unclean}/\Delta r_{cleaned}$ gives an indication of whether the cleaning has been a worthwile exercise in the removal of the systematic.
\begin{table}[!hbp]
\caption{The improvement to the uncertainty in tensor to scalar ratio when cleaning is applied for various levels of gain mismatch.} \label{tab:r values}
\centering
\begin{tabular}{c|c|c}
    Gain Mismatch & $\Delta r_{unclean} / \Delta r_{cleaned}$\\
    &&\\
    \hline
    \hline
    \\
    $0.01$ & $59.6$
    \\
    $0.001$ & $...$
    \\
    $0.0001$ & $...$
    \\
\end{tabular}
\end{table}
Table \ref{tab:r values} shows the effect of the cleaning in the presence of various levels of differential gain.
\NM{We would need to calculate these using the spectra before and after cleaning. This would offer a direct comparison to the Yadav values which would show the difference between the improvements you would likely get with their approximated systematics approach and our realistic scan strategy systematics. Also it would possibly be a good thing for us to have a quantification of the effect on the uncertainty on r measurements regardless of the comparison, although maybe it would be enough to just have the plot in figure \ref{fig:cleaned BB} showing the improvement at power spectrum level?}

==> sections/properties.tex <==




\section{Properties of the Quadratic Estimator}
\label{sec:results}
\subsection{Mode choice}
As seen in section \ref{sec:qe}, when reconstructing the temperature to polarisation leakage it is possible to use information from a range of different CMB modes. It is possible, for example, to perform the reconstruction using only one set of modes (e.g. the EB cross-modes are most commonly used in the reconstruction of anisotropic birefringence), or to use a combination of several different sets of modes. In figure \ref{fig:mode_comparison} we plot the reconstruction noise for the different possible mode choices ($TE$,$EE$,$TB$,$EB$) in order to compare the quality of reconstruction it is possible to achieve using each of the sets of modes. Using equations \eqref{eqn:reconstruction noise for gamma E} and \eqref{eqn:reconstruction noise for gamma B}, these noise values were calculated for an experiment with a beam and noise levels comparable to the projected values for the \emph{LiteBIRD} satellite \cite{Hazumi2019}. 
\par 
It is clear from this comparison that $TB$ cross modes offer the lowest noise reconstruction. 
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_test_EB_noise_gamma_EandB_noisecomparison_Lmax_100_lmax_500.pdf}
    \caption{\NM{MLB - Call the reconstruction noise power spectra something more sensible e.g. $N_L^{\gamma_E \gamma_E}$ etc.}The reconstruction noise power spectra of the $\gamma^{E}_L$ and $\gamma^{BB}_{L}$ temperature to polarisation leakage terms when no temperature to polarisation leakage is present. This figure shows the reconstruction noises for the $EE$ modes (magenta), $TE$ modes (red), $EB$ modes (blue), $TB$ modes (green), and the combination of all the modes (black dots). The reconstruction noise was calculated for maps with a Gaussian white noise of $\omega_p^{-1/2} = 2.7\mu \text{K arcmin}$ and a beam width of $\theta_{FWHM}=0.5^{\circ}$ in analogy to the projected noise and beam profiles for LiteBIRD. The noise curves were calculated for a reconstruction using modes of $\ell \leq 500$.}
    \label{fig:mode_comparison}
\end{figure}
Moreover, we see that using a combination of modes will offer very little improvement over using the $TB$ modes alone. While figure \ref{fig:mode_comparison} shows the reconstruction noise when no leakage is present, if this systematic is present the $TB$ modes still provide the lowest variance reconstruction of the temperature to polarisation leakage. This is also true in the cosmic variance limited case. Therefore, only information from the $TB$ modes will be used in subsequent reconstructions of the temperature to polarization leakage presented in this work.

\subsection{Masked Sky}
There are a number of issues in reality meaning that the use of the full sky in CMB surveys is unviable. A major foreground to CMB observations is caused by galactic emission and as such it is common practice to apply a galactic mask, to remove the worst of these effects from the data. Additionally in the case of ground-based observatories the full sky is not readily available due to their locations on earth, as such smaller patches of the sky are observed often more frequently to aid in achieving a deeper survey to control noise. As such it is important to consider the effects of a masked sky on any estimators devised, since the spin-zero mask field can pose further complications causing additional mode mixing.


Since it is a systematic sourced signal we are considering it is worth noting that the mask is automatically included in the distortion field since any masked pixel will contribute zero systematic. As such the window function of the survey is included in the orientation function (see equation \ref{eqn:h_k}) and is incorporated for all $k$ (for further discussion on this see \cite{2020arXiv200800011M}). Comparing terms in equation \ref{eqn:Signal} it is clear that the $(\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})$ field necessarily includes the window function of the survey. As such the QE considered in this work are equally applicable to the masked sky, with only some degradation due to the smaller sky coverage leaving fewer modes available for the reconstruction. This in essence means for the systematic considered here we could equally apply the QE to ground-based surveys since they are robust in the presence masking. We present results of the QE in the presence of a galactic mask to demonstrate this.






==> sections/qe.tex <==
\section{Quadratic estimators}
\label{sec:qe}
As discussed in section \ref{sec:recap} in this paper we consider a temperature to polarisation leakage induced by a gain mismatch between detectors. The nature of the temperature to polarization leakage, and indeed all of the distortions considered in \eqref{eqn:Distortion Fields}, as perturbative terms makes it possible to reconstruct these fields using quadratic estimators. This is in analogy to lensing reconstruction, where quadratic estimators are applied to the CMB fields to reconstruct the lensing potential \cite{2003PhRvD..68h3002H}

\subsection{Off diagonal correlations}
Normally all correlations between two harmonic space CMB fields, for example the auto-correlation of the $E$-mode polarization $\ensave{E_{lm}E^{*}_{l'm'}}$ or the cross-correlation between the temperature and $E$-mode polarization fields $\ensave{T_{lm}E^{*}_{l'm'}}$, are on diagonal.\NM{MLB Comment - Is this true also on the cut sky? } That is, for these correlations only terms where $l=l'$ are non-zero. This is true for all Gaussian random variables.
However, distortions of the real space primordial CMB fields can lead to off diagonal correlations between the harmonic space fields, where $l\neq l'$ terms are also non-zero.
\par 
In the case of the specific distortion we consider in this paper, the temperature and polarization leakage is treated as a small spin-2 correction to the complex Stokes parameters of the form

\begin{equation}\label{eqn:Stokes Parameter Perturbation}
    {}_{\pm}P(\hat{\mathbf{n}}) + {}_{\pm}\delta P(\hat{\mathbf{n}}) = (\Tilde{Q}\pm i\Tilde{U})(\hat{\mathbf{n}}) + (\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})\Tilde{T}(\hat{\mathbf{n}})\;.
\end{equation}
In this work $\gamma^{Q}$ and $\gamma^{U}$ are  the $Q$ and $U$ like components of the spin-2 temperature to polarization leakage field respectively and are constructed from the product of the gain systematic and the scan. In a realistic case our data model is such that
\begin{equation}
    d = X*B + G\cdot (T*b) + N\;
\end{equation}
Here $X$ represents the polarization maps, $*$ represents a convolution with the beams $B$ for the polarization beam and $b$ for the temperature beam, $G$ represents the temperature to polarization leakage fields, the $\cdot$ represents a multiplication, and N represents the noise.
A perturbation to the stokes parameters will propagate through the $E$ and $B$ mode polarisation decomposition giving additional corrections to the $E$ and $B$ mode harmonic space fields. Details of how these perturbations propogate can be found in appendix \ref{app:QE appendix}. The corrections to $E$ are
\begin{equation}
    \label{eqn:delta elm gamma E}
    \delta E_{lm} = \sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{E}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{equation}
for $l+L+l_{2} =$ even, and
\begin{equation}
    \label{eqn:delta elm gamma B}
    \delta E_{lm} =
    -i\sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{B}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{equation}
for $l+L+l_{2} =$ odd. The corrections to $B$ are
\begin{eqnarray}
    \label{eqn:delta blm gamma E}
    \delta B_{lm} =
    i\sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{E}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,
\end{eqnarray}
for $l+L+l_{2} =$ odd, and
\begin{eqnarray}
    \label{eqn:delta blm gamma B}
    \delta B_{lm} = \sum_{LM}\sum_{l_{2}m_{2}}\gamma_{LM}^{B}\tilde{T}_{l_{2}m_{2}}\xi^{LM}_{lml_{2}m_{2}}\mathcal{H}^{L}_{ll_{2}}\;,\;,
\end{eqnarray}
for $l+L+l_{2} =$ even.
Here $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ are are related to $\gamma^{Q}(\hat{\mathbf{n}})$ and $\gamma^{U}(\hat{\mathbf{n}})$ through a spin-2 spherical harmonic transformation in analogy to the transformation between the $E_{lm}$ and $B_{lm}$ fields and the $Q(\hat{\mathbf{n}})$ and $U(\hat{\mathbf{n}})$ fields. The $\xi^{LM}_{lml'm'}$ and $\mathcal{H}^{L}_{ll'}$ are Wigner-3j geometric terms that encode the coupling between modes inherent in the introduction of such additional anisotropic corrections to the harmonic space fields. The exact forms of the geometric terms are found in appendix \ref{app:QE appendix}. 
\par 
Such corrections to the $E_{lm}$ and $B_{lm}$ manifest themselves in the off diagonal auto- and cross-correlations between the harmonic space fields. The anisotropic systematics introduce a degree of statistical anisotropy that lead to correlations in the off diagonal. One can see off diagonal correlations if, for example, one takes the cross correlations between the $T_{lm}$ and $B_{lm}$ fields. Assuming no primordial $B$-mode polarisation the result is
\begin{equation}\label{eqn:deltaB T cross gamma B}
    \left\langle B_{lm}T^{*}_{l'm'}\right\rangle = \sum_{LM}\gamma_{LM}^{B}\tilde{C}^{TT}_{l'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'} \;,
\end{equation}
for $l+L+l' =$ even, and 
\begin{equation}\label{eqn:deltaB T cross gamma E}
    \left\langle B_{lm}T^{*}_{l'm'}\right\rangle = i\sum_{LM}\gamma_{LM}^{E}\tilde{C}^{TT}_{l'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'} \;,
\end{equation}
for $l+L+l' =$ odd. Here, we discard any terms that are higher than first order in $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$, as these are expected to be small. Tilde symbols are used denote that a given $C_{l}$ is the power spectrum for a primordial CMB field. As the primordial, on diagonal contributions to $\left\langle B_{lm}T^{*}_{l'm'}\right\rangle$ are zero, both \eqref{eqn:deltaB T cross gamma B} and \eqref{eqn:deltaB T cross gamma E} contain only on- and off-diagonal anisotropic contributions from the temperature to polarization leakage distortion.

\subsection{Estimating the distortion} 
It is possible to use the presence of additional statistical anisotropy and off diagonal terms in the correlations between the harmonic space fields in order to estimate the distortion fields $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ This is done by inverting \eqref{eqn:deltaB T cross gamma B} and \eqref{eqn:deltaB T cross gamma E}. For simplicity we collect the terms in \eqref{eqn:deltaB T cross gamma B} into $J^{LM,',XX'}_{ll'}$ and the terms in \eqref{eqn:deltaB T cross gamma E} into $K^{LM,',XX'}_{ll'}$ where,
\begin{equation}J^{LM,',XX'}_{ll'}\equiv\gamma^{B}_{LM}Z^{XX'}_{ll'}\;,
\end{equation}
and 
\begin{equation} 
K^{LM,',XX'}_{ll'}\equiv\gamma^{E}_{LM}\zeta^{XX'}_{ll'}\;.
\end{equation}
The definitions of $Z^{XX'}_{ll'}$ and $\zeta^{XX'}_{ll'}$ for a given choice of $XX'$ can be seen in table \ref{tab:Z values}. 
\begin{table}[!htp]
\caption{Table of $Z^{L,\,A}_{ll'}$ and $\zeta^{L,\,A}_{ll'}$ along with the with the parity for which the terms are required to be non-zero.\label{tab:Z values}}
    \centering
    \begin{tabular}{c|cc|cc|}
     $XX'$ & $Z^{A}_{ll'}$ & parity requirements & $\zeta^{A}_{ll'}$ & parity requirements\\
     &&&&\\
     \hline
     \hline
     &&&&\\
     $BT$ & $C^{TT}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ even & $-iC^{TT}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ odd\\ 
     &&&&\\
     $TB$ & $C^{TT}_{l}H^{L}_{ll'}$& $l+l'+ L =$ even & $iC^{TT}_{l}H^{L}_{ll'}$ & $l+l'+ L =$ odd \\
     &&&&\\
     $BE$ & $C^{TE}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ even & $-iC^{TE}_{l'}\mathcal{H}^{L}_{ll'}$ & $l+l'+ L =$ odd \\
     &&&&\\
     $EB$ & $C^{TE}_{l}H^{L}_{ll'}$ & $l+l'+ L =$ even & $iC^{TE}_{l}H^{L}_{ll'}$ & $l+l'+L =$ odd\\
     &&&&\\
     $EE$ & $i(C^{TE}_{l'}-C^{TE}_{l})$ & $l+l'+ L =$ odd& $C^{TE}_{l} + C^{TE}_{l'}$  & $l+l'+ L =$ even\\
\end{tabular}
\end{table}
It is possible to write estimators for  $J^{LM,',XX'}_{ll'}$ and $K^{LM,',XX'}_{ll'}$ in terms of the observed CMB fields, the exact detail of how this is done is seen in appendix \ref{app:QE appendix 2}. It is then merely a matter of dividing these anisotropic terms by any unwanted terms in order to give $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$. That is, for a given set of multipoles $ll'$ and choice of fields $XX'$ (shortened to $A$),
\begin{eqnarray}
    (\widehat{\gamma}^{B}_{LM})^{A}_{ll'} =&&\, \frac{\widehat{J}^{LM,\,A}_{ll'}}{F^{L,\,A}_{ll'}}\;,\label{eqn:gamBhat}\\
    (\widehat{\gamma}^{E}_{LM})^{A}_{ll'} =&&\, \frac{\widehat{K}^{LM,\,A}_{ll'}}{\mathcal{F}^{L,\,A}_{ll'}}\;.\label{eqn:gamEhat}
\end{eqnarray}
Here, the hats on $\widehat{J}^{LM,\,A}_{ll'}$ and $\widehat{K}^{LM,\,A}_{ll'}$ indicate that they are the estimators. Moreover, the terms that are divided through are defined as  $F^{L,\,A}_{ll'}\equiv Z^{A}_{ll'}W_{l}W_{l'}$ and $\mathcal{F}^{L,\,A}_{ll'}\equiv \zeta^{A}_{ll'}W_{l}W_{l'}$ and contain the beam window function $W_{l}$. Inverse variance weighting can be used to move from an estimate for a given multipole pair and choice of $A$ to a full averaged estimate. This inverse variance weighted average takes the form 
\begin{equation}\label{eqn:gamma E estimator}
    \widehat{\gamma}^{E}_{LM} = \mathcal{N}^{E}_{L}\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}\mathcal{F}^{L,A'}_{ll'}\widehat{K}^{LM,\,A}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\;,
\end{equation}
where and $\mathcal{C}^{ll'}_{AA'}$ is the covariance matrix for the covariance of $\widehat{K}^{LM,\,A}_{ll'}$ and 
\begin{equation}
    G^{L}_{ll'} = \frac{(2l+1)(2l'+1)}{4\pi}\;.
\end{equation}
Here, $\mathcal{N}^{E}_{L}$ represents the reconstruction noise for the estimator and is included due to the inverse variance weighting. It is calculated as follows:
\begin{equation}\label{eqn:reconstruction noise for gamma E}
    \mathcal{N}^{E}_{L} = \left(\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}\mathcal{F}^{L,\,A}_{ll'}\mathcal{F}^{L,\,A'}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\right)^{-1}\;.
\end{equation}
The full estimator for $\gamma^{B}_{LM}$ has the similar form 
\begin{equation}\label{eqn:gamma B estimator}
    \widehat{\gamma}^{B}_{LM} = \mathcal{N}^{B}_{L}\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}F^{L,A'}_{ll'}\widehat{J}^{LM,\,A}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\;,
\end{equation}
and
\begin{equation}\label{eqn:reconstruction noise for gamma B}
    \mathcal{N}^{B}_{L} = \left(\sum_{l'\geq l}G^{L}_{ll'}\sum_{AA'}F^{L,\,A}_{ll'}F^{L,\,A'}_{ll'}\left[(\mathcal{C}^{ll'})^{-1}\right]_{AA'}\right)^{-1}\;.
\end{equation}

The summation over $l$ is limted to $l\leq l'$ to avoid over counting as under the exchange of indices $l\leftrightarrow l'$ the exchange of fields $XX' \leftrightarrow X'X$ occurs. One does not need such measures if the estimator is limited to using either $XX'$ or $X'X$. However, this is less efficient in harmonic space than using both $XX'$ and $X'X$ with the limited $l$ range.

\subsection{Efficient estimators}
\par
Due to the presence of the Wigner-3j symbol containing geometric terms these estimators are very computationally demanding, scaling as $\sim l^{4}$.  It is possible to write the estimators of specific combinations of modes, for example $TB$ only. This is beneficial as some combinations of modes perform better than others, often performing so well that using more than one combination of modes is unnecessary. Moreover, using fewer mode combinations requires less computing time. However, to further reduce computing time it is also necessary to rewrite these estimators in a way that avoids calculating a large number of Wigner-3j symbols. As these estimators involve a convolution in harmonic space they can be written as simple products of the real space fields, thus avoiding computing any Wigner-3j symbols. We begin by writing the estimators that only use the $TB$ modes,
\begin{equation}
    \widehat{\gamma}^{B}_{LM} = 
    \mathcal{N}^{B}_{L}\sum_{l l'mm'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'}\frac{B_{lm}T^{*}_{l'm'}}{C^{BB,\,\rm map}_{l}C^{TT,\,\rm map}_{l'}}\tilde{C}^{TT}_{l'}W_{l}W_{l'}\;,
\end{equation}
where $l+l'+L= {\rm even}$ and
\begin{equation}
    \widehat{\gamma}^{E}_{LM} = -i\mathcal{N}^{E}_{L}\sum_{l l'mm'}\xi^{LM}_{lml'm'}\mathcal{H}^{L}_{ll'}\frac{B_{lm}T^{*}_{l'm'}}{C^{BB,\,\rm map}_{l}C^{TT,\,\rm map}_{l'}}\tilde{C}^{TT}_{l'}W_{l}W_{l'}\;,
\end{equation}
where $l + l' + L = {\rm odd}$. Note that we have not limited sum over $l$ to $l\leq l'$. Limiting the range of the sum is unnecessary in the case of the efficient estimators as this sum is never explicitly carried out.
The reconstruction noises for these TB only estimators are
\begin{equation}\label{eqn:TB noise B}
    \mathcal{N}^{B}_{L} = \sum_{l'\geq l}(1+\delta_{ll'})^{-1}G^{L}_{ll'}\left[\frac{\left|F^{L,BT}_{ll'}\right|^{2}}{C^{BB,\,\rm map}_{l}C^{TT\,\rm map}_{l'}} + \frac{\left|F^{L,TB}_{ll'}\right|^{2}}{C^{TT,\,\rm map}_{l}C^{BB\,\rm map}_{l'}}\right]\;,
\end{equation}
and,
\begin{equation}
    \mathcal{N}^{E}_{L}= \sum_{l'\geq l}(1+\delta_{ll'})^{-1}G^{L}_{ll'}\left[\frac{\left|\mathcal{F}^{L,BT}_{ll'}\right|^{2}}{C^{BB,\,\rm map}_{l}C^{TT\,\rm map}_{l'}} + \frac{\left|\mathcal{F}^{L,TB}_{ll'}\right|^{2}}{C^{TT,\,\rm map}_{l}C^{BB\,\rm map}_{l'}}\right]\;.
\end{equation}
We do not write reconstruction noise in a more efficient form so the limit $l\leq l'$ still applies when calculating $\mathcal{N}^{B}_{L}$ and $\mathcal{N}^{E}_{L}$. In principle $C^{\rm map}_{l} = W^{2}_{l}\tilde{C}_{l} + C^{\,\rm noise}_{l}$, where $C^{\,\rm noise}_{l}$ is the noise power spectrum, and $W_{l}$ is the beam window function given by $W_{l} \approx \exp(-l^{2}\sigma_{b}^{2}/2)$ with $\sigma_{B} = \Theta_{\rm FWHM}/\sqrt{8\ln2}$ \cite{Kamionkowski1997a}. However, in practice $C^{\rm map}_{l}$ must be directly estimated from the polarization maps as their values are effected significantly by the presence of the temperature to polarization leakage.  $C^{\rm map}_{l} = \tilde{C}_{l} + C^{\,\rm noise}_{l}$. The geometric kernel terms $\xi^{LM}_{lml'm'}$ and $\mathcal{H}^{L}_{ll'}$ can be written as real space integrals of spin weighted spherical harmonics. When this is done, taking into account the difference in parity between the two estimators one arrives at the efficient estimators,
\begin{eqnarray}
    \widehat{\gamma}^{B}_{LM} =&&\,\frac{\mathcal{N}^{B}_{L}}{2}\int d\hat{\mathbf{n}}\big[{}_{-2}Y_{LM}(\hat{\mathbf{n}}){}_{-2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\nonumber\\ 
    &&\,+ {}_{+2}Y_{LM}(\hat{\mathbf{n}}){}_{+2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\big]\;,
\end{eqnarray}
and 
\begin{eqnarray}
    \widehat{\gamma}^{E}_{LM} =&&\,\frac{-i\mathcal{N}^{E}_{L}}{2}\int d\hat{\mathbf{n}}\big[{}_{-2}Y_{LM}(\hat{\mathbf{n}}){}_{-2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\nonumber\\ 
    &&\,- {}_{+2}Y_{LM}(\hat{\mathbf{n}}){}_{+2}(A_{B^{*}}(\hat{\mathbf{n}}))^{*}A_{T^{*}}^{TT}(\hat{\mathbf{n}})\big]\;.
\end{eqnarray}
Here the real space fields are written as transforms of the harmonic space $E_{lm}$ and $B_{lm}$ terms in the following forms:
\begin{eqnarray}
    {}_{s}A_{X}(\hat{\mathbf{n}}) =&&\, \sum_{lm}\frac{1}{C^{XX}_{l}}X_{lm}{}_{s}Y_{lm}(\hat{\mathbf{n}})\;,\\
    {}_{s}A^{XY}_{X'}(\hat{\mathbf{n}}) =&&\, \sum_{lm}\frac{\tilde{C}_{l}^{XY}}{C^{X'X'}_{l}}X'_{lm}{}_{s}Y_{lm}(\hat{\mathbf{n}})\;,
\end{eqnarray}


==> sections/recap.tex <==
\section{Distortion Fields}
\label{sec:recap}
In the ideal scenario the true CMB polarisation signal would be isolated and easily measurable. However in reality it is subject to a plethora of contaminants. A number of these contaminants can be characterised by their spin dependence and as such readily written in to a set of distortion fields.


The work of \cite{2010PhRvD..81f3512Y} and \cite{2003PhRvD..67d3004H} describe the effects of various cosmological signals and systematic effects on the measured polarisation at map level through 11 distortion fields as
\begin{eqnarray}
    {}_{\pm}\delta P(\hat{\mathbf{n}}) &&= [a \pm i 2\omega](\hat{\mathbf{n}}){}_{\pm}P(\hat{\mathbf{n}}) + [f_{1} \pm if_{2}](\hat{\mathbf{n}}){}_{\mp}P(\hat{\mathbf{n}}) + [\gamma_{1} \pm i\gamma_{2}](\hat{\mathbf{n}})\tilde{T}(\hat{\mathbf{n}})
    \nonumber\\
    &&+\sigma \mathbf{{}_{1}p}(\hat{\mathbf{n}}) \cdot {}_{\mp}\nabla {}_{\pm}P(\hat{\mathbf{n}};\sigma) + \sigma [d_{1} \pm id_{2}](\hat{\mathbf{n}}) [\partial_{1} \pm i\partial_{2}]\tilde{T}(\hat{\mathbf{n}};\sigma) +\sigma^{2}q(\hat{\mathbf{n}})[\partial_{1} \pm i\partial_{2}]^{2}\tilde{T}(\hat{\mathbf{n}};\sigma) + ...
    \label{eqn:Distortion Fields}
\end{eqnarray}
where ${}_{\pm}P(\hat{\mathbf{n}}) = \tilde{Q} \pm \tilde{U}$ is the spin-2 polarisation and ${}_{\pm}\delta P(\hat{\mathbf{n}})$ corresponds to some correction to the polarisation field. It is worth noting here that the form of these distortion fields will be highly dependent on the scanning strategy and as such a realistic scan should be employed when considering drawing conclusions. We look at this in detail in section \ref{sec:Realistic Scan}.


Equation \ref{eqn:Distortion Fields} has been constructed such that the top line corresponds to mixing between polarisation and temperature in a known direction on the sky. While the bottom line considers mixing in a local region with some directional dependence such that they leak the derivative of the CMB fields, e.g. pointing or lensing. The length scale $\sigma$ corresponding to the width of a Gaussian beam that is smoothing the CMB fields. The second line quantities are sourced by a simple first order Taylor expansion of the CMB fields around $\hat{\mathbf{n}}$, however a number of first order contaminants have been neglected in this equation which we shall explore in section \ref{sec:Additional Terms}.


Since ${}_{\pm}P$ is a spin $\pm2$ field the distortions to this must be spin $\pm2$ also, this necessitates that $a(\hat{\mathbf{n}})$ and $\omega(\hat{\mathbf{n}})$ are scalar fields describing an amplitude scaling and a polarisation plane rotation respectively, $[f_{1} \pm if_{2}](\hat{\mathbf{n}})$ is a spin $\pm 4$ field which couples the conjugate polarisation fields, $[\gamma_{1} \pm i\gamma_{2}](\hat{\mathbf{n}})$ is a spin $\pm2$ field that couples the temperature to polarisation directly. $\mathbf{{}_{1}p}(\hat{\mathbf{n}}) = {}_{1}[p_{1} \pm ip_{2}](\hat{\mathbf{n}})$ is a spin $\pm1$ deflection field that describes direction changes of the photons, $[d_{1} \pm id_{2}](\hat{\mathbf{n}})$ is a spin $\pm1$ field and $q(\hat{\mathbf{n}})$ is a scalar field that couple the first and second derivatives of the temperature field to the polarisation respectively. Since there are no known processes that cause T to P conversion along the line of sight each of the T containing terms can be attributed to some systematic.



Each of the terms in equation \ref{eqn:Distortion Fields} may be attributed to some cosmological signal or systematic. We will not provide an exhaustive list here but will pick out some important terms to explore. It is indicated in \citep{2010PhRvD..81f3512Y} that the $(\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})$ field poses the largest B-mode contaminant. As such we have chosen to concentrate on this field which hereafter we relabel $(\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})$ in analogy with the stokes parameters. The source of this particular field which leaks temperature to polarisation can be attributed to a differential gain systematic. Indeed, the distortion fields we focus on in this work are the differential gain that induce temperature to polarization leakage. While we choose a specific distortion, we do this with the aim of demonstrating cleaning and reconstruction techniques that could be more generally applicable to the full list of distortions seen in equation \eqref{eqn:Distortion Fields}.


\subsection{Additional Terms}
\label{sec:Additional Terms}
Some additional terms that contribute to the distortion field, that were neglected in equation \ref{eqn:Distortion Fields} sourced from \citep{2010PhRvD..81f3512Y} include
\begin{eqnarray}
\label{eqn:Additional Distortion Terms}
    {}_{\pm}\delta P^{\text{New}}(\hat{\mathbf{n}}) &&= \sigma \mathbf{{}_{-1}p}(\hat{\mathbf{n}}) \cdot {}_{\pm}\nabla {}_{\pm}P(\hat{\mathbf{n}};\sigma) + \sigma \mathbf{{}_{3}p}(\hat{\mathbf{n}}) \cdot {}_{\pm}\nabla {}_{\mp}P(\hat{\mathbf{n}};\sigma) + \sigma \mathbf{{}_{5}p}(\hat{\mathbf{n}}) \cdot {}_{\mp}\nabla {}_{\mp}P(\hat{\mathbf{n}};\sigma)
    \nonumber\\
    &&+ \sigma \mathbf{{}_{3}d}(\hat{\mathbf{n}}) [\partial_{1} \mp i\partial_{2}]\tilde{T}(\hat{\mathbf{n}};\sigma) + \sigma^{2} \mathbf{{}_{4}q}(\hat{\mathbf{n}})[\partial_{1} \mp i\partial_{2}]^{2}\tilde{T}(\hat{\mathbf{n}};\sigma).
\end{eqnarray}
These additional terms correspond to additional leading order terms in the Taylor expansion that describe the directional dependent contaminants of equation \ref{eqn:Distortion Fields}. It is important not to neglect these terms as there are a number of systematics that would result in these distortion fields being non-zero. We point out in particular that a differential pointing systematic, which would contribute to the terms containing the $[d_{1} \pm id_{2}](\hat{\mathbf{n}})$ and $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$ field in equation \ref{eqn:Distortion Fields}, also contributes to a number of other terms in equation \ref{eqn:Additional Distortion Terms}. This includes additional coupling of the conjugate of the derivative of the Temperature field with the Polarisation through the spin-3 $\mathbf{{}_{3}d}(\hat{\mathbf{n}})$ field, which through examining figure \ref{fig:Distortion Fields} it is clear contributes a systematic of similar level to the spin-1 contribution and as such should not be neglected. In addition the differential pointing will also contribute to the terms containing the fields $\mathbf{{}_{-1}p}(\hat{\mathbf{n}})$, $\mathbf{{}_{5}p(\hat{\mathbf{n}})}$, and $\mathbf{{}_{3}p(\hat{\mathbf{n}})}$ which induce polarisation mixing as detailed in \cite{2020arXiv200800011M}. With the unprecedented sensitivity levels planned for future CMB missions it is more important than ever to understand the systematics present, and not neglect any of the terms that could bias measurements.


\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/DistortionFields.pdf}
    \caption{The left column shows maps of the spin-2 $(\gamma_{1}+i\gamma_{2})(\hat{\mathbf{n}})$ distortion field sourced by a 1\% differential gain systematic which causes a T leakage into the polarisation. The second and third columns show the spin-1 $({}_{1}d_{1}+i{}_{1}d_{2})(\hat{\mathbf{n}})$ and spin-3 $({}_{3}d_{1}+i{}_{3}d_{2})(\hat{\mathbf{n}})$ distortion fields sourced by a $0.1'$ differential pointing systematic which causes a leakage of the derivative of the temperature into the polarisation. These fields have been calculated analytically using the product of the appropriate spin scan field and the systematic as explained in section \ref{sec:Differential Gain} with further information available in \cite{2020arXiv200800011M}.  There is clearly significant difference between the distortion fields sourced by different systematics, though the structure of the scan is visible in all. This demonstrates that taking into account the scan strategy for such systematics is pivotal to fully understand the viability of methods to reconstruct systematics. Note that the spin 1 and 3 fields of the middle and right panels are of a similar magnitude suggesting each will contribute a comparable level of differential pointing systematic which is not negligible.}
    \label{fig:Distortion Fields}    
\end{figure}


%\subsection{Issues for Lensing Estimators}
%\AR{We can skip these details for this paper. We can have a brief discussion on this when we present perspectives. This doesnt fit in to other details we discuss in this paper.}
%When travelling from the surface of last scattering to us the CMB photons are subjected to deflections by the intervening matter. This effect known as weak gravitational lensing causes a redistribution of the CMB photons and may be written as \cite{1998PhRvD..58b3003Z,2003PhRvD..68h3002H,2005PhRvD..71l3527C}
%\begin{eqnarray}
%    {}_{\pm}\delta P(\hat{\mathbf{n}}) &&= {}_{\pm}P(\hat{\mathbf{n}} + \nabla \Phi + \nabla \times \Omega)\nonumber
%    \\
%    &&= \nabla \Phi \cdot \nabla {}_{\pm}P(\hat{\mathbf{n}}) + \nabla \times \Omega \cdot \nabla {}_{\pm}P(\hat{\mathbf{n}}) + ...
%\end{eqnarray}
%where the second line has been written using the Taylor expansion about $\hat{\mathbf{n}}$. The deflection field $\nabla \Phi$ is sourced by linear order density perturbations in the intervening matter where $\Phi$ is the projected gravitational potential along the line of sight. While the $\nabla \times \Omega$ deflection field would be sourced by higher order scalar gravitational potentials (e.g. deflection by multiple lenses along the line of sight) or by exotic non-$\Lambda$CDM matter (e.g. topological defects). The curl part is usually much smaller than the grad and is generally treated as vanishingly small. However there is a further source that can contribute to both the grad and curl components, a contamination from systematics.



%The deflection field $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$ included in equation \ref{eqn:Distortion Fields} is attributed to the effect of lensing when considered in \citep{2010PhRvD..81f3512Y}. The gradient term $\nabla \Phi$ contributes to the $p_2(\hat{\mathbf{n}})$ deflection field and the curl term is contained in $p_1(\hat{\mathbf{n}})$ deflection field. However fields of this form can also be sourced by a number of systematics, which as such could cause a bias when attempting lensing reconstruction. The work of \cite{2005PhRvD..71l3527C} for instance advocates using the presence of a curl component as systematic diagnostic.


%We point out here in particular that, as shown in \cite{2020arXiv200800011M}, the form of the differential pointing systematic means it could mimic both the grad and curl parts of lensing. We already noted that a T-P coupling is generated by the differential pointing systematic, however the differential pointing will also contribute as a deflection field acting on the polarisation directly and as such will contaminate the lensing contribution to the deflection field $\mathbf{{}_{1}p}(\hat{\mathbf{n}})$. This is an important observation to make as consequently the presence of a differential pointing systematic could interfere with the QE used to reconstruct CMB lensing and vice versa. Furthermore this excess signal from differential pointing could in principle cause an overestimation of the lensing amplitude parameter $A_{lens}$ \cite{2008PhRvD..77l3531C}. As the differential pointing contributes to other terms in equations \ref{eqn:Distortion Fields} and \ref{eqn:Additional Distortion Terms} that the CMB lensing signal does not, it could in principle be possible to combine the QE for these fields along with prior information of the scan strategy to disentangle the systematic from the lensing signal. We leave this to further work to explore in detail.





==> sections/reconstructionold.tex <==
\section{Optimal filtering for cleaning and reconstruction}

\subsection{Map and power spectrum reconstruction with map filtering}
The efficient form of the quadratic estimators are applied to the CMB Temperature map, $T(\uvec{n})$, and polarization maps, $Q(\uvec{n})$ and $U(\uvec{n})$ produced by the simulations described in \ref{sub:Simulation}. The resulting reconstructed harmonic space temperature to polarization leakage fields, $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$, must be filtered so that modes that are saturated by reconstruction noise are down-weighted in comparison to high signal to noise ratio (SNR) modes. We define SNR at each multipole, $L$, as 
\begin{equation}
    \text{SNR}_{L} = \frac{\widehat{C}^{\gamma^{\chi\chi}}_{L}-\mathcal{N}^{\chi}_{L}}{\sqrt{\frac{2}{2L+1}}\mathcal{N}^{\chi}_{L}}\;,
\end{equation}
where $\widehat{C}^{\gamma^{\chi\chi}}_{L}$ is the estimator for the power-spectum of either $\gamma^{E}_{LM}$ or $\gamma^{B}_{LM}$, defined as 
\begin{equation}
    \widehat{C}^{\gamma^{\chi\chi}}_{L} \equiv \sum_{M=-L}^{L}\frac{\left|\widehat{\gamma}^{\chi}_{LM}\right|^{2}}{2L+1}
\end{equation}
Our filter is constructed so that
\begin{equation}
F^{\chi\chi}_{L} = \begin{cases}
    0, & \text{if SNR}_{L} \leq 1\\
    A\exp\left(-\left[\frac{\widehat{C}^{\gamma^{\chi\chi}}_{L}}{\widehat{C}^{\gamma^{\chi\chi}}_{L}-\mathcal{N}^{\chi}_{L}}\right]^{2}\right),&\text{if SNR}_{L} > 1\\
\end{cases}\;.
\label{eqn:filter}
\end{equation}
The filter is normalized by $A$ so that the maximum value the filter will take is $F^{\chi\chi}_{L} = 1$. These filters are applied in harmonic space to the $\gamma^{E}_{LM}$ and $\gamma^{B}_{LM}$ fields. These fields are transformed to the real space, $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$, fields.
\par 
In figure \ref{fig:map comparisons} we compare the resulting filtered, reconstructed temperature to polarization leakage maps, $\gamma^{Q}(\uvec{n})$ and $\gamma^{U}(\uvec{n})$, to the actual leakage maps calculated directly from the input differential gain and prior knowledge of the scan, and to the actual leakage fields with only information up the $L_{\rm max}$ of the reconstructed fields.
\par 
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_hybrid_real_multiplot_map_Lmax_1000_lmax_3000.pdf}
    \caption{A comparison of the true systematic maps (left) and the systematic maps reconstructed up to $L=1000$ using an efficient quadratic estimator (right). Also presented here is the true systematic map with multipole information of $L>1000$ removed (center). The noise and beam for the simulated maps are chosen to emulate the proposed \textit{LiteBIRD} experiment \cite{Hazumi2019}.}
    \label{fig:map comparisons}    
\end{figure}
The features of the input leakage maps are correctly reconstructed. When comparing the reconstructed maps to the input maps only in the range the reconstruction was performed over we see that the amplitudes of the reconstructed maps match the input maps. The amplitude of the full input maps is larger than the reconstructed due to the extra power coming from the modes above $L_{\rm max}$.
\par 
The efficacy of the reconstruction and the importance of filtering is better seen in a comparison between the power spectra of the true and \emph{unfiltered} reconstructed systematic maps; such a comparison can be seen in figure \ref{fig:ps comparisons}. 
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/nialh_hybrid_real_gamma_EandB_powspec_Lmax_1000_lmax_3000_iter_0.pdf}
    \caption{A comparison of the true $C^{\gamma^{EE}}_{L}$ and $C^{\gamma^{BB}}_{L}$ power spectra (blue dots) and the $\widehat{C}^{\gamma^{E}}_{L}$ and $\widehat{C}^{\gamma^{B}}_{L}$ quadratic estimator reconstructed power spectra (orange dots) in the range $2\leq L\leq1000$ with no filtereing applied. The noise and beam for the simulated maps are chosen to emulate the proposed \textit{LiteBIRD} experiment \cite{Hazumi2019}. It can be seen that the reconstruction noise (red) becomes dominant at $L\sim50$ for both sets of power spectra. \NM{MLB Comment - Need to make very clear that although the reconstruction noise is dependent on the signal, this is not a problem because you measure the reconstruction noise (in addition to the "signal + noise" power directly from the map. (This currently doesn't come across at all in either the main text or the caption.) (Comment applies to this figure, and the associated discussion in the text in section D.)}}
    \label{fig:ps comparisons}    
\end{figure}
Note that in the $L$ range below $L=50$ the power spectra of the input maps and unfiltered, reconstructed maps match. However, the reconstruction noise becomes dominant at $L\sim 50$ and it is impossible to effectively reconstruct the systematic maps at these higher multipoles. That is, at the smaller scales corresponding to these higher multipoles the reconstructed maps will be dominated by the reconstruction noise. These are the modes that must be down-weighted through filtering in order to give a leakage map that is not heavily biased by the reconstruction noise.

\subsection{Reconstructing different levels of differential gain}

We run the simulation described in section \ref{sub:Simulation} for $\delta g_{1} = \delta g_{2} = $ 0.01, 0.001, and 0.0001. We show the $\widehat{C}^{\gamma^{EE}}_{L}$ and $\widehat{C}^{\gamma^{BB}}_{L}$ power spectra recovered from the unfiltered, reconstructed maps, the reconstruction noise, and $C^{\gamma^{EE}}_{L}$ and $C^{\gamma^{BB}}_{L}$ from the input maps for all three gain levels in figure \ref{fig:gain levels}.
\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figures/diff_gain_comp_nonoise_gamma_EandB_powspec_Lmax_100_lmax_500.pdf}
    \caption{Reconstructed $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$ spectra and reconstruction noise for a 1\% (orange) , 0.1\% (red), and 0.01\% (magenta) differential gain. The input $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$ spectra are also displayed in blue, green and black for the 1\%, 0.1\% and 0.01\% differential gain respectively.}
    \label{fig:gain levels}    
\end{figure}
\par 
For all three levels of differential gain the quality of reconstruction appears to be similar, with a similar maximum $L$ at which the reconstruction is not dominated by noise. The amplitude of the reconstruction noise appears to be proportional to the level of systematic included in the scan. This is to be expected as the variance of the observed CMB power spectra $C_{l}^{TT}$ and $C_{l}^{BB}$ feeds directly into the covariance matrix for the quadratic estimator. Therefore, a systematic which increases the variance of these spectra will increase the covariance for the quadratic estimator and therefore increase the reconstruction noise for $\gamma^{EE}_{L}$ and $\gamma^{BB}_{L}$. 
\par 
We also performed this study keeping $\delta g_{1}$ and $\delta g_{2}$ fixed but allowing $w^{-1/2}_p$ to take the values in the range $w^{-1/2}_p=0\mu\text{K-arcmin}$ to $w^{-1/2}_p=5\mu\text{K-arcmin}$. Changing the pixel noise resulted in different levels of reconstruction noise. However, the change in reconstruction noise is small, and has only a small effect on the $L$ at which the reconstruction noise becomes dominant. The $L$ at which the noise saturates the reconstruction is only a factor of $\sim2$ less for $w^{-1/2}_{p} = 5\mu\text{K-arcmin}$ than for $=w^{-1/2}_{p}\mu\text{K-arcmin}$. The input differential gain has a much more profound effect on amplitude of the reconstruction noise.
\par
The quadratic estimator technique can be used as an excellent tool to diagnose temperature to polarization leakage in CMB maps without prior knowledge of the instrument or scan because it is possible to reconstruct even very low levels of temperature to polarization leakage effectively. For all three levels of differential gain there is a maximum $L$ beyond which the reconstruction noise dominates. However, below this multipole it is possible to precisely reconstruct the temperature to polarization leakage systematic.

==> sections/simulations_preDan.tex <==
\section{\label{sec:T to P Sims}Simulating Temperature to Polarization Leakage}
\subsection{Systematic - Differential Gain\label{sec:Differential Gain}}
\JW{eqref all the refs} 
In upcoming experiments, both satellite- and ground-based, control of T to P leakage will be essential. The relative amplitudes of the signals means that even temperature leakage at the percent level could be a significant contaminant to B-mode science goals. This section will describe the simulation of T to P leakage we have chosen and briefly explain the scan strategy we consider, though in principle the methods outlined are applicable to a wider range of distortions to the maps generated by systematic effects in the instrument.

\JW{is this repetitive}

\JW{maybe also refer to distortion field}

In principle, the QE method may be tailored for use on any systematic sourced map level distortion that varies across the sky. Here, we will present the specific details of how a differential gain in a detector pair in the instrument can source a T to P leakage map level distortion. Understanding this is vital for producing realistic simulations of this systematic effect for the case study we are examining. 
\par 
The signal observed by a single detector contains both the temperature and modulated polarisation signals and may be written as
\begin{equation}
    d^X = (1+g^X) (\tilde{T}(\hat{\mathbf{n}}) + \tilde{Q}(\hat{\mathbf{n}})\cos(2\psi) + \tilde{U}(\hat{\mathbf{n}})\sin(2\psi))\;,
\end{equation}
where $g^X$ represents the offset from the true signal due to some gain miscalibration in the detector, $X$ denotes which detector is being considered, and $\psi$ is the crossing angle (orientation of the focal plane on the sky).

We consider a pair-differencing experiment which relies on co-located detector pairs oriented 90 degrees apart to decouple. Ideally the temperature signal would be completely removed by this procedure. However, any mismatches in the detectors will result in leakage of the temperature signal into the polarisation.


We write the differenced signal as 
\begin{eqnarray}
    d_i =&& \frac{1}{2}d^A_i - d^B_i
    \nonumber\\
    =&& \frac{1}{2} \bigg[(g^{A}_i-g^{B}_i)\tilde{T}(\hat{\mathbf{n}})
    +\tilde{Q}(\hat{\mathbf{n}})[(1+g^A_i)\cos(2\psi) - (1+g^B_i)\cos(2\psi+\pi)] 
    \nonumber\\
    &&+\, \tilde{U}(\hat{\mathbf{n}})[(1+g^A_i)\sin(2\psi) - (1+g^B_i)\sin(2\psi+\pi)]\bigg]
    \nonumber\\
    =&&\frac{1}{2}\bigg[(g^A_i-g^B_i)\tilde{T}(\hat{\mathbf{n}}) + \tilde{Q}(\hat{\mathbf{n}})[2+g^A_i+g^B_i]\cos(2\psi)\nonumber\\
    &&+\, \tilde{U}(\hat{\mathbf{n}})[2+g^A_i+g^B_i]\sin(2\psi)\bigg]\;,
\end{eqnarray}
where $A$ and $B$ denote each detector in the co-located pair, and $i$ denotes which pair they belong to. The temperature leakage will dominate in the case of the $B$-mode spectrum, so we neglect polarisation terms and write the spurious polarisation signal due to differential gain in a single detector pair as
\begin{equation}
    \delta d^g_i = \frac{\delta g_i}{2} \, \tilde{T}(\hat{\mathbf{n}})\;,
    \label{eqn:DiffGain}
\end{equation}
where the gain mismatch is given by $\delta g_i = g^{A}_i-g^{B}_i$.


It is the contribution of this spurious signal to the spin-2 polarisation field that is of interest, however the spurious temperature term from the differential gain of equation~\eqref{eqn:DiffGain} is clearly a spin-0 quantity. We, therefore, require further information from the scanning strategy to determine how this spin-0 contaminant is coupled to the spin-2 polarisation signal. We may describe a given scanning strategy by a real space field given by
\begin{equation}
h(\psi, \theta, \phi)=\frac{2\pi}{N_{\text{hits}}}\sum_j \delta(\psi-\psi_j(\theta,\phi))\;,
\end{equation}
where $\psi_j$ is the $j$th crossing angle of a given pixel, and $N_{\text{hits}}$ is the total number of crossings of that pixel. This orientation function has mixed spin-weight and can be expanded as a Fourier series as
\begin{equation}
    \tilde{h}_k = \frac{1}{N_{\text{hits}}(\theta, \phi)} \sum_{j} e^{ik\psi_j(\theta, \phi)}\;,
    \label{eqn:h_k}
\end{equation}
where $\tilde{h}_0$ describes the survey's window function, while the other spins can be used when determining systematic effects \cite{2009arXiv0906.1188B,2017MNRAS.466..425W,2020arXiv200800011M}. We may use this to write the total spin-2 signal detected within a pixel in Fourier space as a convolution,
\begin{equation}
    \tilde{S}^{d}_{2}(\Omega) = \sum_{k'=-\infty}^{\infty}\tilde{h}_{2-k'}(\Omega)\tilde{S}_{k'}(\Omega)\;,
\end{equation}
where $\tilde{S}^{d}_{2}(\Omega)$ is the total spin-2 signal, and $\tilde{S}_{k'}(\Omega)$ is the spin-$k'$ signal being coupled to this by the relevant scan term. In the case of equation~\eqref{eqn:DiffGain}, we see that the field in question is the spin-0 temperature field multiplied by some spin-0 differential gain component and we may rewrite the equation for a single detector pair as
\begin{equation}
    {}_2(\delta d^g_i) = \frac{1}{2} \tilde{h}_2(\hat{\mathbf{n}}) (\delta g_i) \, \tilde{T}(\hat{\mathbf{n}})\;.
\end{equation}


In this work we consider a focal plane two co-located pairs of detectors oriented at 45 degrees to one another to allow simultaneous measurement of both $\tilde{Q}$ and $\tilde{U}$ signals. It is the spin-2 signal that we are interested in and the combined systematic contribution to the observed signal of the two detectors is thus given by
\begin{equation}
{}_2(\delta d^g) = \frac{1}{2} \tilde{h}_2(\hat{\mathbf{n}}) (\delta g_1 - i\delta g_2) \, \tilde{T}(\hat{\mathbf{n}})
\label{eqn:Spin2Signal}
\end{equation}
where the factor of $i$ in the second detector term is due to the rotated orientation of 45 degrees.


For simplicity we choose a setup where each pair of the detectors experiences the same differential gain, $\delta g_1 = \delta g_2 = 0.01$, which corresponds to a 1\% differential gain. This simplification will not affect the generality of the QE results presented, but one may expect slightly different levels of gain mismatch for different focal plane setups. %The gain will also modify the polarisation signal directly by an amplification of the of the true signal which leads to essentially a monopole increase of the spectrum, which we choose to remove post process. 
Therefore, we only consider the T to P term of equation~\eqref{eqn:Distortion Fields} when writing the estimator which relates to the systematic as
\begin{equation}
\begin{split}
(\gamma^{Q}\pm i\gamma^{U})(\hat{\mathbf{n}})\Tilde{T}(\hat{\mathbf{n}}) = \frac{1}{2} \tilde{h}_{\pm 2}(\hat{\mathbf{n}}) (\delta g_1 \mp i\delta g_2) \, \tilde{T}(\hat{\mathbf{n}})\;.
\end{split}
\label{eqn:Signal}
\end{equation}


\subsection{Scan Strategy}
\label{sec:Scan Strategy}
We choose to adopt the Experimental Probe of Inflationary Cosmology (\textit{EPIC}) satellite scan strategy \citep{2009arXiv0906.1188B}. This will representative of other future CMB satellite surveys. The design of the EPIC scan strategy optimises crossing angle coverage and is defined by its boresight angle ($50^\circ$), precession angle ($45^\circ$), spin period (1 min), and precession period (3 hrs) (for further details see \cite{2017MNRAS.466..425W} and \cite{2008arXiv0805.4207B}).

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/EPICHITMAP.pdf}
    \caption{The hit map of the \textit{EPIC} scan strategy. This survey has been designed to maximise crossing angle coverage, and the hit map is well filled across the full sky with many observations at different orientations. Note that the galactic poles have been prioritised to aid the understanding of foregrounds and galactic science goals hence the higher number density in the hit map in those regimes}
    \label{fig:Hit Map}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/ScanMaps.pdf}
    \caption{The real (left panel) and imaginary (right panel) parts of the $\tilde{h}_2$ field (defined in equation \ref{eqn:h_k}), which encodes the spin-2 part of the scan that turns the gain systematic into a spurious spin-2 signal. The $\tilde{h}_2$ field is dominated by its large scale features, which will result in a low $l$ dominated systematic.}
    \label{fig:Scan Maps}
\end{figure}


The scan strategy of \textit{EPIC} provides a relatively uniform distribution of hits and crossing angles which should reduce scan coupled differential systematics fairly well. The galactic poles are observed more frequently to aid in foreground analysis and galactic science goals, which results in some structure appearing in the survey fields as seen in Figure~\ref{fig:Hit Map}. The $\tilde{h}_{\pm 2}$ field (equation~\eqref{eqn:h_k}) encodes the spin-2 part of the scan that turns the gain systematic into a spurious spin-2 signal. This field is shown in Figure~\ref{fig:Scan Maps} for the \textit{EPIC} scan strategy. The $\tilde{h}_2$ is dominated by its large scale features, and this will result in a low $l$ dominated systematic.


\subsection{Simulation\label{sub:Simulation}}
The input to the time ordered data (TOD) simulation code consists of maps of the CMB $\tilde{T}$, $\tilde{Q}$ and $\tilde{U}$ fields which are generated using the {SYNFAST} routine of the {HEALPIX} package \citep{2005ApJ...622..759G}. The input CMB power spectra were created in CAMB using a six parameter $\Lambda$CDM cosmological model, specified in Table~\ref{tab:simulation inputs} \cite{Lewis:1999bs}. We use a Gaussian beam representative of the \emph{LiteBIRD} effective beam \cite{Hazumi2019}. For the simulations including noise, this we include this post process. A white noise is applied to the data at map level, where a noise is added to each pixel of the level $w_{TT}^{-1} = 2.7\mu \text{K arcmin}$ \citep{2019JLTP..194..443H}.
\begin{table}[h!]
    \centering
    \begin{tabular}{cl}
    \hline\hline
        &Simulation Inputs\\
        \hline\hline
         Cosmology & $H_{0}$ = 67.4\\
         &$\Omega_{b}h^{2} = 0.022$\\
         &$\Omega_{c}h^{2} = 0.120$\\
         &$\tau = 0.06$\\
         &$n_{s} = 0.97$\\
         &$10^{9}A_{s} = 2.2$\\
         &$r = 0.001$\\
         \hline
         Map-making &$N_{\rm side} = 2048$\\
         &$\ell_{\rm max} = 3000$\\
         &$|\delta g_{1}| = 0.01$\\
         &$|\delta g_{2}| = 0.01$\\
         \hline
    \end{tabular}
    \caption{The fiducial cosmological parameters and the map-making inputs for the TOD simulations. The simulated maps are smoothed by a Gaussian beam and noise is added per pixel.}
    \label{tab:simulation inputs}
\end{table}


%
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/GammaEEComparison.pdf}
    \caption{The E-mode spectrum of the ${}_{\pm}\gamma(\uvec{}n)$ distortion fields, the orange and green lines show the spectra plotted for the $A_{D}^{\text{Max}}$ amplitudes of \citep{2010PhRvD..81f3512Y} for coherences scales of $10^{\prime}$ and $120^{\prime}$ respectively, the red and purple lines show the spectra plotted for the $A_{D}^{\text{Min}}$ amplitudes of \citep{2010PhRvD..81f3512Y} for the CMBPol satellite estimate corresponding to r=0.005 for coherences scales of $10^{\prime}$ and $120^{\prime}$ respectively. The blue line shows the realistic spectrum calculated from the a combination of the systematic and the \emph{EPIC} scan strategy that we adopt for our simulations. It is clear here that the approximation used for the distortion power spectra does not describe the realistic case well at higher multipoles. It overestimates the power at high multipoles in comparison to the realistic case for small coherence scales. Additionally the sharp drop off in power after the peak is not consistent with the realistic spectra as is evident for all sets of curves showing the approximation.}
    \label{fig:Realistic Gamma Comparison}    
\end{figure}
%



%The TOD simulation is setup to perform a pair-differencing experiment using co-located detector pairs oriented 90 degrees apart. We consider two co-located pairs of detectors oriented at 45 degrees to one another to allow simultaneous measurement of both $\tilde{Q}$ and $\tilde{U}$ signals. 
The simulation computes values for each of the four detectors for each hit, using HEALPIX interpolation to observe the input sky maps at the appropriate location. For each hit the simulation uses the corresponding parallactic angle for that hit, generated from the \textit{EPIC} scan strategy, to compute the detected value as
\begin{equation}
d^X_i = \tilde{T}(\hat{\mathbf{n}}) +  \tilde{Q}(\hat{\mathbf{n}})\cos{(2\psi)} + \tilde{U}(\hat{\mathbf{n}})\sin{(2\psi)}\text{,}
\end{equation}
where the $\psi$ values are offset by $90^\circ$ for the two detectors within a pair (labelled by $X$), and by $45^\circ$ between the two pairs of detectors (labelled by $i$). The differential gain systematic is added for each pair of detectors by increasing the signal by a factor $(1-\delta g_{i})$ in the second detector $d^B_i$ in each pair, where we use $|\delta g_{1}| = |\delta g_{2}| = 0.01$ for the simulations in this work \citep{2020MNRAS.491.1960T}. This level of systematic is indicative of the differential gain seen in recent CMB surveys \citep[e.g.][]{2015ApJ...814..110B,1403.2369}.


Maps are made from the time streams according to a simple binning map making technique,
\begin{equation}
\begin{pmatrix}Q\\U\end{pmatrix}
=
\begin{pmatrix}\langle \cos^{2}(2\psi_{i}) \rangle&\langle \cos(2\psi_{i})\sin(2\psi_{i}) \rangle\\\langle \sin(2\psi_{i})\cos(2\psi_{i}) \rangle&\langle \sin^{2}(2\psi_{i}) \rangle\end{pmatrix}^{-1}
\begin{pmatrix}\langle d_{i}\cos(2\psi_{i}) \rangle\\\langle d_{i}\sin(2\psi_{i}) \rangle\end{pmatrix}\;,
\label{eq:2x2 map making}
\end{equation}
where the angle brackets $\langle \rangle$ denote an average over the measurements in a pixel, and the $d_j$ here corresponds to the detector measurement each of which has an associated angle $\psi_j$. %However, in the presence of a gain mismatch between the detectors within a pair this can result in the differential gain leaking the much larger temperature signal into the polarisation data.


\subsection{Realistic Systematic Spectra}
\label{sec:Realistic Scan}
In previous studies \citep[e.g.][]{2003PhRvD..67d3004H,2010PhRvD..81f3512Y} the distortion fields of equation \ref{eqn:Distortion Fields} have been assumed to be statistically isotropic and Gaussian, and defined by power spectra of the form
\begin{equation}
    C_{l}^{DD} = A_{D}^{2} e^{-l(l+1)\sigma_{D}^{2}/8\ln{2}}\;,
    \label{eqn:Syst Cl Approx}
\end{equation}
where $A_D$ represents the root mean squared of the distortion field, and $\sigma_{D}$ represents some coherence scale beyond which the distortion power spectrum becomes white noise.  There are significant differences apparent between the approximation of equation \ref{eqn:Syst Cl Approx} for the power spectra describing the distortion fields used in previous literature, and the realistic distortion field that is derived from the more realistic simulation used in our study.


Although the spectrum generated from equation \ref{eqn:Syst Cl Approx} results in most of the power being at low multipoles similar to the realistic spectra, it does not capture the high $l$ nature of the realistic distortion fields. The realistic distortion fields have an initial much sharper drop off, before levelling out, compared to the more gradual drop off of the approximation. In figure \ref{fig:Realistic Gamma Comparison} we show that the two extreme coherence scales used in \citep{2010PhRvD..81f3512Y} both suffer from the same issue that they accrue too much power at high $l$ compared to the realistic spectra, hence the results found will be biased by this. In our analysis in Section~\ref{sec:reconstruction} we reconstruct the distortion power spectrum up to $L=800$ and, as can be seen in figure \ref{fig:Realistic Gamma Comparison}, the difference in shape between the realistic and approximate spectra differs significantly for this range of multipoles.
This shows the advantage of carrying out detailed case studies on individual distortions.
\par 
We note  that the smallest  $A_D^{\rm min} \approx %4.8\times10^{-4},
1.3\times10^{-4}$ for $\sigma_{D}=%10^{\prime},
120^{\prime}$ quoted from \cite{2010PhRvD..81f3512Y} corresponds to a gain mismatch of $%2.4\times10^{-3} (0.24\%),
6.4\times10^{-4} (0.064\%)$. This is significantly smaller than a realistic gain mismatch of 0.01 (1\%), in the analysis in \cite{2010PhRvD..81f3512Y} it was found that the QE technique would still be effective for this small value of the systematic.

==> sections/todo.tex <==
\section{Comments and to do's}
\subsection{General}
\begin{enumerate}
    \item \NM{Yadav uses EB as it is optimal under their assumptions, point out this is not true for our realistic take.}
    
    \item \NM{Yadav is flat sky, point out explicitly the improvement in that we have full sky and optimal estimators.}
    
    \item \NM{Yadav eqn 19 assumes flat white noise like spectrum for the gamma spectra, point out how this differs in our realistic case.}
    
    \item \NM{Yadav signal-noise plots motivates our choice of exploring the gammas since they are largest effect in their case, add this somewhere.}

    \item \NM{Add galactic masked plots.}
    
    \item \NM{Add different beams plots.}
    
    \item \NM{Add different gain levels plots.}

    \item These methods are generic to diffuse mapping experiments and have applicability to beyond CMB measurements.
    
    \item \AR{An exercise we can try is to use the foreground contaminated sky at say 100 GHz, and then try to pass it through TOD to map, and then run the QE on it just the same, except, we use the map power spectrum, to see if it will at all work in the presence of foregrounds. My strong suspicion is that it will not as foregrounds are stongly anisotropic and the QE makes an assumption about the isotropy of the background field. {\bf THIS IS A LOW PRIORITY TASK.}}
    
    \item \AR{{\bf This we should try to make our analysis seem more realistic.} We can run the EB QE on masked skies. Since the E and B fields are not correlated except due to the systematic, I think this might work and we wont have to worry about the bias subtraction of the systematic. The bias one can show is zero for the EB estimator. However when measuring the primordial B-mode power spectrum we will need to introduce additional machinery to correct for the E to B power leakage due to masking. I have the machinery to do this and we can certainly think of pushing in this direction to make the analysis look more realistic.}
\end{enumerate}

\subsection{Specific Sections}
\begin{enumerate}
    \item Quadratic estimators - \AR{Summarize only the main results here. Sketch the derivation in the appendix. We don't need to provide each step of the derivation, just the important steps involved.}
    
    \item  Results - \AR{ Measurement of the systematics maps and comparison with inverting the systematics introducing procedure -- the true systematics maps. Measurement of the gain mismatch of the detectors, compare versus true gain, make assessment of the quality of the recovery. De-systematize the B-mode map, show map level comparison if interesting. Show power spectra with systematics and without systematics. Show corrected B-mode power spectrum recovery for different Lmax construction of the systematics. }
    
    \item Simulating Temperature to Polarization Leakage - \AR{EPIC scan details. Noise details. gain mis match details. Disscuss differences from the notation used in the Yadav paper. Show example maps. Maybe differences between simulated maps and ideal data, to show how small are the map level systematics!! what sets the amplitude of the systematics and why are the values we have injected reasonable? Why are we focusing on this particular systematic, does this have a speacial bearing on upcoming measurements of the microwave sky?}
\end{enumerate}
